Spingarn's Method and Progressive Decoupling Beyond Elicitable Monotonicity

Spingarn's method of partial inverses and the progressive decoupling algorithm address inclusion problems involving the sum of an operator and the normal cone of a linear subspace, known as linkage problems. Despite their success, existing convergence results are limited to the so-called elicitable monotone setting, where nonmonotonicity is allowed only on the orthogonal complement of the linkage subspace. In this paper, we introduce progressive decoupling+, a generalized version of standard progressive decoupling that incorporates separate relaxation parameters for the linkage subspace and its orthogonal complement. We prove convergence under conditions that link the relaxation parameters to the nonmonotonicity of their respective subspaces and show that the special cases of Spingarn's method and standard progressive decoupling also extend beyond the elicitable monotone setting. Our analysis hinges upon an equivalence between progressive decoupling+ and the preconditioned proximal point algorithm, for which we develop a general local convergence analysis in a certain nonmonotone setting.

==> TeX/Text/DRS/connection.tex <==
%!TEX root = ../../../ProgDec-Minty.tex
Consider the composite inclusion problem
\begin{equation}\label{prob:linkage-DRS}
    \text{find} \quad x \in \R^n \quad \text{such that} \quad 0 \in S(x) + N_X(x). \tag{P-DRS}
\end{equation}
Then, given a positive stepsize $\gamma$ and relaxation parameter $\lambda$, the (relaxed) Douglas--Rachford splitting method consists of the following iterates.
\begin{equation}
    \begin{cases}\tag{DRS}\label{eq:DRS}
        \displaystyle   
        x^k&= \proj_X(s^k)\\
        q^k&\in J_{\gamma^{-1} S}(2x^k-s^k)\\
        s^{k+1}&=s^k+\lambda(q^k-x^k).
    \end{cases}
\end{equation}
Consider the change of variable $s^k = x^k - \gamma^{-1}y^k$. It is easy to see from the above updates that 
\[
x^{k+1} 
=
\proj_X(s^{k+1}) 
= 
\proj_X(s^k+\lambda(q^k-x^k)) 
=
\proj_X(x^k - \gamma^{-1}y^k + \lambda(q^k-x^k)),
\]
and that 
\[
y^{k+1} 
  = 
\gamma(x^{k+1} - s^{k+1})
    =
\gamma(x^{k+1} - s^k - \lambda(q^k-x^k))
    =
y^k + \gamma(x^{k+1} - (1- \lambda)x^k - \lambda q^k).
\]
Changing the order of updates in \eqref{eq:DRS} by starting from \(q^k\) update, and using the above relations, it can be equivalently formulated as 
\begin{equation}
    \begin{cases}\label{eq:DRS:2}
        \displaystyle   
        q^k&\in J_{\gamma^{-1} S}(x^k + \gamma^{-1}y^k)\\
        x^{k+1}&= 
        \proj_X(x^k - \gamma^{-1}y^k + \lambda_k(q^k-x^k))\\
        y^{k+1} &= 
        y^k + \gamma(x^{k+1} - (1- \lambda)x^k - \lambda_kq^k).
    \end{cases}
\end{equation}
If the algorithm is initialized with \(x^0 \in X\), \(y^0 \in X^\bot\), then it reduces to
\begin{equation}
    \begin{cases}\label{eq:DRS:PD}
        \displaystyle   
        q^k&\in J_{\gamma^{-1} S}(x^k + \gamma^{-1}y^k)\\
        x^{k+1}&= 
        (1-\lambda) x^k + \lambda\proj_X(q^k)\\
        y^{k+1} &= 
        y^k - \gamma\lambda \proj_{X^\bot}(q^k)
    \end{cases}
\end{equation}
This is an instance of \eqref{eq:progdec} with \(\lambda_x = \lambda_y\). The next proposition shows that the underlying semimonotonicity assumption from \Cref{ass:progdec-local} corresponds to the existence of $\DRSRho$\hyp{}weak Minty solutions of the so-called primal-dual inclusion, where 
\(
  \DRSRho
    {}={} 
  \blkdiag(\com \proj_X, \mon \proj_{X^\bot})
\).
Note that in \cite{evens2023convergence} the setting where 
\(
  \DRSRho
    {}={} 
  \blkdiag(\com \I_n, \mon \I_n)
\)
was previously studied for DRS.
The proof can be found in \Cref{proof:prop:partialinverse:implications}
\begin{proposition}\label{prop:partialinverse:implications}
  Let \(X \subseteq \R^n\) be a closed linear subspace. Consider the operator \(S : \R^n \rightrightarrows \R^n\) and suppose that the partial inverse \(S^X\) has a $\DRSRho$\hyp{}weak Minty solution at $u^\star \in \zer S^X$, where \(V = \mon \proj_{X^\bot}+\com \proj_X \).
  Then, the following hold.
  \begin{enumerate}
      \item \label{it:partialinverse:implications:semi} Operator $S$ is $(\mon \proj_{X^\bot}, \com \proj_{X})$\hyp{}semimonotone at $\bigl(\proj_X(u^\star), \proj_{X^\bot}(u^\star)\bigr)$.
      \item \label{it:partialinverse:implications:WMVI} The primal-dual operator 
      \(
          \Tpd : (x,y) \mapsto \begin{bmatrix}
              N_X(x) + y\\
              S^{-1}(y) - x
          \end{bmatrix}
      \) has a $\blkdiag(\com \proj_X, \mon \proj_{X^\bot})$\hyp{}oblique weak Minty solution at $\bigl(\proj_X(u^\star), \proj_{X^\bot}(u^\star)\bigr) \in \zer \Tpd$.
  \end{enumerate}
\end{proposition}

==> TeX/Text/Examples/H-levelsets.tex <==
\begin{example}
    Let $a \coloneqq \tfrac{11}4$ and consider the minimization problem
    \begin{align*}
        &&\minimize_{x \in \R^3}&
        \quad
        f(x) = \tfrac12\left(1+x_3\right)\left(x_1^2 + x_2^2\right) - a \csc(2a)\sin^2(x_1)\cos^2(x_2) - \tfrac12\sqrt{1 + x_1^2x_2^2}\\
        \quad
        &&\stt&
        \quad
        x \in X \coloneqq \set{x \in \R^3}[x_3 = 0].
    \end{align*}
    \begin{proof}
        It holds that
        \begin{align*}
            \nabla f(x)
                {}={}
            \begin{bmatrix}
                (1 + x_3)x_1 - a\csc(2a)\sin(2x_1)\cos^2(x_2) + \tfrac{x_1x_2^2}{2\sqrt{1 + x_1^2x_2^2}}\\
                (1 + x_3)x_2 + a\csc(2a)\sin^2(x_1)\sin(2x_2) + \tfrac{x_1^2x_2}{2\sqrt{1 + x_1^2x_2^2}}\\
                \tfrac12\left(x_1^2 + x_2^2\right)
            \end{bmatrix}
        \end{align*}
        and
        \begin{align*}
            \nabla^2 f(x)
                {}={}
            \begin{bmatrix}
                1 + x_3 + 2a\csc(2a)\cos(2x_1)\cos^2(x_2) + \tfrac{x_2^2}{2(1 + x_1^2x_2^2)\sqrt{1 + x_1^2x_2^2}} &
                a\csc(2a)\sin(2x_1)\sin(2x_2) + \tfrac{x_1x_2(1+x_1^2x_2^2)}{2(1 + x_1^2x_2^2)\sqrt{1 + x_1^2x_2^2}}
                & x_1\\
                a\csc(2a)\sin(2x_1)\sin(2x_2) + \tfrac{x_1x_2(1+x_1^2x_2^2)}{2(1 + x_1^2x_2^2)\sqrt{1 + x_1^2x_2^2}} &
                1 + x_3 + 2a\csc(2a)\sin^2(x_1)\cos(2x_2) + \tfrac{x_1^2}{2(1 + x_1^2x_2^2)\sqrt{1 + x_1^2x_2^2}} &
                x_2\\
                x_1 & x_2 & 0
            \end{bmatrix}
        \end{align*}
        Let
        $
            N = \set{x \in X}[|x_1| \leq \tfrac32]
        $.
        This seems like a good example for weak Minty. Inspired by examples in paper by Gower from 2021. Maybe not good for this work though.
    \end{proof}
\end{example}

==> TeX/Text/Examples/VonNeumann.tex <==

\begin{example}[Von Neumann's economic equilibrium model]\label{ex:VonNeumann}
    Using the standard definition of the simplex
    \(
    \Delta_d \coloneqq \set{z \in \R^d}[ z \geq 0, \sum_{i=1}^d z_i = 1]
    \),
    consider an economy where there are 
    $n$ goods with relative prices $y \in \Delta_n$,
    which can be produced by $m$ processes with relative intensities $x \in \Delta_m$.
    Let $R_{ij} \geq 0$ and $S_{ij} \geq 0$ denote the number of units of the $j$th good produced and consumed by the $i$th process, respectively.
    % Assume that the total value of all goods produced is strictly positive, i.e., that $\inner{x, Sy} > 0$ for all $x \in \Delta_m$, $y \in \Delta_n$.
    By \cite[\S 5]{neumann1945model}, a pair $(x^\star, y^\star)$ for which this economy is expanding corresponds to a minimax solution of
    % there exist intensities $x^\star$ and prices $y^\star$ such that the economy is expanding if and only if there exists a saddle point solution to the minimax problem
    \begin{align*}
        \minimize_{x \in \Delta_m} 
        \;
        \maximize_{y \in \Delta_n} 
        \;
        f(x,y) \coloneqq \frac{\inner{x, Ry}}{{\inner{x, Sy}}}.
        \numberthis\label{eq:ex:neumann}
    \end{align*}
    Defining $z \coloneqq (x, y)$, the problem of finding stationary points of \eqref{eq:ex:neumann} corresponds to finding a zero of
    \[
        T(z)
            {}\coloneqq{}
        F(z)
        +
        N_C(z),
    \]
    where
    $
        F(z)
            {}={}
        \begin{psmallmatrix}
            \nabla_x f(x,y) \\
            - \nabla_y f(x,y)
        \end{psmallmatrix}
        % \left(\nabla_x f(x,y), - \nabla_y f(x,y)\right)
    $
    and 
    $
        C = \Delta_2 \times \Delta_2
    $.
    Denote the vector of all $1$s of dimension $n$ by $\mathbf{1}_n$ and let
    $
        \tilde z 
            \coloneqq 
        % (x - \tfrac1d \mathbf{1}_d, y - \tfrac1d \mathbf{1}_d)
        z - \tfrac1d \mathbf{1}_{2d}
    $.
    Then, this problem is equivalent to finding a zero of
    \[
        \tilde T(\tilde z)
            \coloneqq
        T(\tilde z + \tfrac1d \mathbf{1}_{2d})
            {}={}
        F(\tilde z + \tfrac1d \mathbf{1}_{2d})
            +
        N_C(\tilde z + \tfrac1d \mathbf{1}_{2d})
            {}={}
        \underbrace{
        \tilde F(\tilde z)
            +
        N_{\set{\tilde z \,\geq\, -\nicefrac1d}}(\tilde z)}_{\eqqcolon\, \tilde S(\tilde z)}
            +
        N_X(\tilde z)
    \]
    where
    \(
        X
            {}\coloneqq{}
        \set{(\tilde x, \tilde y) \in \R^{2d}}[\sum_{i=1}^d \tilde x_i = 0, \sum_{i=1}^d \tilde y_i = 0]
    \),
    which is equivalent to the linkage problem
    \begin{equation}
        \text{find} \quad (\tilde z, \tilde v) \in \R^{2d} \times \R^{2d} \quad \text{such that} \quad \tilde z \in X, \quad \tilde v \in X^{\bot},\quad \tilde v \in \tilde S(\tilde z).
    \end{equation}
    Let $\varepsilon \in (0,1)$ and let
    \begin{align*}
        R 
            {}={} 
        \begin{bmatrix}
            0 & 1 + \nicefrac{\varepsilon}2\\
            2 - \nicefrac{\varepsilon}2 & 2
        \end{bmatrix}
        \quad\text{and}\quad
        S
            {}={}
        \begin{bmatrix}
            \nicefrac12 & \nicefrac12\\
            1 & 1
        \end{bmatrix}.
        \numberthis\label{eq:prop:ex:neumann:matrices}
    \end{align*}
    \begin{proof}
        By \cite[Ex. 2.7]{evens2023convergence}, we know that the unique Nash equilibrium 
        $
            z^\star
                \coloneqq
            (x^\star, y^\star) =
            \begin{bsmallmatrix}
                0 & 1 & 0 & 1
            \end{bsmallmatrix}^\top
        $
        of \eqref{eq:ex:neumann} is a $\Bigl(\tfrac{\varepsilon-1}{4}\Bigr)$\hyp{}weak Minty solution of $T$.
        Consequently, it follows from \cite[Prop. 4.4]{evens2023convergence} that 
        $
            \tilde z^\star 
                =
            z^\star - \nicefrac12\mathbf{1}_{4}
                =
            \begin{bsmallmatrix}
                -\nicefrac12 & \nicefrac12 & -\nicefrac12 & \nicefrac12
            \end{bsmallmatrix}^\top
        $
        is a $\Bigl(\tfrac{\varepsilon-1}{4}\Bigr)$\hyp{}weak Minty solution of $\tilde T$. 
        
    \end{proof}

\end{example}

==> TeX/Text/Examples/decomposable.tex <==
Suppose that the operator $S : \R^n \rightrightarrows \R^n$ can be decomposed as
\[
    S(x) = S(x_1,\hdots,x_q) = \bigl(S_1(x_1),\hdots,S_q(x_q)\bigr) \quad\text{for mappings}\quad S_i : \R^{n_i} \rightrightarrows \R^{n_i}.
\]
where $n = \sum_i=1^q n_i$.
Then, linkage problem \eqref{prob:linkage-intro} reduces to 
\begin{equation}
    \label{prob:linkage-decomposable}
    \text{find}\quad
        (x_1,\hdots,x_q) \in X
    \quad\text{and}\quad 
        (y_1,\hdots,y_q) \in X^\bot
    \quad\text{such that}\quad 
        y_i\in S_i(x_i) 
    \quad\text{for all}\quad
        i = 1,\hdots,q.
    % \tag{P-decomposable}
\end{equation}
and the first step of \ref{eq:progdec} can be performed in parallel, since
\begin{equation*}
    q^k = (q_1^k,\hdots,q_q^k)
        \quad\text{where}\quad
    q_i^k \in J_{\gamma^{-1} S_i}(x_i^k + \gamma^{-1}y_i^k)    
        \quad\text{for all}\quad
    i = 1,\hdots,q.
\end{equation*}
In the optimization setting of \eqref{prob:linkage-optimization}, when
\[
    \psi(x) = \psi(x_1,\hdots,x_q) = \psi_1(x_1)+\hdots+\psi_q(x_q) \quad\text{for lsc functions}\quad \psi_i : \R^{n_i} \rightarrow \Rinf.
\]
then under suitable constraint qualifications the first-order optimality conditions are given by \eqref{prob:linkage-decomposable}, with $S_i = \partial \psi_i$. Then, the first step of \ref{eq:progdec} corresponds to solving
\begin{equation}\label{eq:linkage-decomposable-optim:q-step}
    % q^k = (q_1^k,\hdots,q_q^k)
    %     \quad\text{where}\quad
	0 \in \partial \psi_i^k(q_i^k) \quad \text{where} \quad 
	\psi_i^k(q_i)
		\coloneqq
	\psi_i(q_i) - \inner{y_i^k, q_i} + \tfrac{\gamma}{2}\nrm{q_i - x_i^k}^2
        \quad\text{for all}\quad
    i = 1,\hdots,q.
\end{equation}
\hl{TODO: When is this an optimization problem?}


==> TeX/Text/Examples/henon-heiles.tex <==

This famous problem provides a mathematical model concerning the chaotic motion of a star in a gravitational field of a galaxy.
If the potential of a particle is larger than the potential of the saddle points, the particle escapes the stable region and goes to infinity.
Therefore, we are interested in both the saddle points and the minima of the potential function.
Relate to bifurcations and cite work of Ferrer.
Relate to the potential energy surface (PES), transition states and maybe also the Müller-Brown PES.

\begin{example}
    Consider the generalized three-dimensional H\'{e}non-Heiles potential
    \begin{align*}
        V(x)
            {}\coloneqq{}
        \tfrac12(a_1x_1^2 + a_2x_2^2 + a_3x_3^2) + (b_1x_1^2 + b_2x_2^2)x_3 - \tfrac{c}{3}x_3^3
    \end{align*}
    Let $x \in X \coloneqq \set{x \in \R^3}[x_2 = 0]$, constraining the potential to a 2-dimensional subspace.
    Let $x^\star$ be the local minimum and $s_i$ be the saddle points. 
    Then, $\nabla f$ is $(\mon \proj_{x^\bot}, \com \proj_X)$-semimonotone on $N_{x^\star} \times \R^3$, and $(\mon \proj_{x^\bot}, \com \proj_X)$-semimonotone on $N_{s_i} \times \R^3$ for $i = 1, 2, 3$.
\end{example}
\begin{proof}
    Note that
    \begin{align*}
        \nabla f(x)
            {}={}
        \begin{bmatrix}
            a_1 x_1 + 2b_1x_1x_3\\
            a_2 x_2 + 2b_2x_2x_3\\
            a_3 x_3 + b_1x_1^2 + b_2x_2^2 - c x_3^2
        \end{bmatrix}
        \quad\text{and}\quad
        \nabla^2 f(x)
            {}={}
        \begin{bmatrix}
            a_1 + 2 b_1 x_3 & 0 & 2 b_1 x_1 \\
            0 & a_2 + 2 b_2 x_3 & 2 b_2 x_2\\
            2 b_1 x_1 & 2 b_2 x_2 & a_3 - 2c x_3
        \end{bmatrix}
    \end{align*}
    If $x_2 = 0$:
    \begin{align*}
        \nabla f(x)
            {}={}
        \begin{bmatrix}
            a_1 x_1 + 2b_1x_1x_3\\
            0\\
            a_3 x_3 + b_1x_1^2 - c x_3^2
        \end{bmatrix}
        \quad\text{and}\quad
        \nabla^2 f(x)
            {}={}
        \begin{bmatrix}
            a_1 + 2 b_1 x_3 & 0 & 2 b_1 x_1 \\
            0 & a_2 + 2 b_2 x_3 & 0\\
            2 b_1 x_1 & 0 & a_3 - 2c x_3
        \end{bmatrix}
    \end{align*}
\end{proof}


==> TeX/Text/Examples/rosenbrock-theory.tex <==

\begin{example}\label{example:Rosenbrock}
    Let $b > 0$ and consider the minimization problem
    \begin{align*}
        \minimize_{x \in \R^3}
        \quad
        f(x) \coloneqq x_1x_2 + b(x_3-x_1^2)^2
        \quad
        \stt
        \quad
        x \in X \coloneqq \set{x \in \R^3}[x_1 = x_2].
        \numberthis\label{eq:example:Rosenbrock}
    \end{align*}
    Then, $\nabla f$ is 
    $\Bigl(-\nicefrac94 \proj_{X^\bot}, -\nicefrac{1}{4}\proj_X\Bigr)$-semimonotone
    at $(x^\star, 0)$, where $x^\star = (0, 0, 0)$ is the global minimum of \eqref{eq:example:Rosenbrock}.
    \begin{proof}
        Note that 
        \begin{align*}
            \nabla f(x)
                {}={}
            \begin{bmatrix}
                x_2 - 4bx_1(x_3 - x_1^2)\\
                x_1\\
                2b(x_3 - x_1^2)
            \end{bmatrix},
            \quad
            \nabla^2 f(x)
                {}={}
            \begin{bmatrix}
                8bx_1 -4bx_3  & 1 & -4bx_1\\
                1 & 0 & 0\\
                -4bx_1 & 0 & 2b
            \end{bmatrix},
            \quad
            \proj_X
                {}={}
            \begin{bmatrix}
                \nicefrac12 & \nicefrac12 & 0\\
                \nicefrac12 & \nicefrac12 & 0\\
                0 & 0 & 1
            \end{bmatrix}
            \quad\text{and}\quad
            \proj_X
                {}={}
            \begin{bmatrix}
                \nicefrac12 & -\nicefrac12 & 0\\
                -\nicefrac12 & \nicefrac12 & 0\\
                0 & 0 & 0
            \end{bmatrix}.
        \end{align*}
        Therefore, $\nabla f$ is 
        $\Bigl(a \proj_{X^\bot}, b\proj_X\Bigr)$-semimonotone
        at $(x^\star, 0)$ if 
        \begin{align*}
            \inner{x - \other{x}, \nabla^2 f(x + \tau(\other{x} - x)) (x - \other{x})} \geq \mon \|\proj_{X^\bot} (x - \other{x})\|^2 + \com \|\proj_X \Bigl(\nabla f(x) - \nabla f(\other{x})\Bigr)\|^2,
            \qquad \forall x, \other{x} \in \R^3, \tau \in (0,1).
        \end{align*}
        Checking this does not seem as easy.
    \end{proof}
\end{example}

\hl{TODO: We need to add examples which use } \Cref{cor:semimon:lin:functions,ex:consensus:cond}

==> TeX/Text/Introduction/contributions.tex <==
%!TEX root = ../../../ProgDec-Minty.tex

% The convergence analyses in both \cite{spingarn1983Partial,rockafellar2019Progressive} relied on casting these methods as particular instances of the (preconditioned) proximal point algorithm (PPPA).
% Specifically, by leveraging established results for PPPA in the maximally monotone setting \cite{martinet1970Regularisation,rockafellar1976Monotone}, their convergence in the (elicitable) monotone setting was demonstrated directly. 
% However, the preconditioned proximal point algorithm is known to converge in more general settings as well. 
% For instance, it was demonstrated that PPPA converges also for maximally comonotone operators \cite{pennanen2002Local,iusem2003Inexact} and operators which admit so-called \emph{weak Minty solutions} \cite{evens2023convergence}.
% Moreover, these works illustrate that PPPA can deal with higher degrees of nomonotonicity when an additional relaxation step is incorporated into the algorithm.

% More recently, \cite{rockafellar2019Progressive} introduced the \emph{progressive decoupling} algorithm, a generalization of Spingarn's method that incorporates an additional stepsize parameter $\gamma$.
% Notably, convergence of this method was established in the \emph{elicitable monotone} setting, i.e., when $S - \mu \proj_{X^{\bot}}$ is maximally monotone for some $\mu < 0$, under the condition that the stepsize satisfies $\gamma > -\mu$.
% In other words, this convergence result demonstrates that this class of methods is capable of solving linkage problems \eqref{prob:linkage-intro} even when $S$ is nonmonotone on the subspace $X^\bot$.

% In this work, we aim to design a simple algorithm for solving linkage problems \eqref{prob:linkage-intro} in the case where $S$ is not necessarily elicitable monotone.
% To this end, we consider a generalized version of the progressive decoupling algorithm for solving~\eqref{prob:linkage-intro} which introduces two additional relaxation parameters $\lambda_{x}$ and $\lambda_{y}$. 
% This algorithm, which we refer to as \emph{progressive decoupling+}, is defined as
% \begin{equation}
% 	\begin{cases}
% 		\displaystyle   
% 		q^k &\in J_{\gamma^{-1} S}(x^k + \gamma^{-1}y^k)\\
% 		x^{k+1}&= (1 - \lambda_{x})x^{k} + \lambda_{x}\proj_X (q^k)\\
% 		y^{k+1}&= y^{k} - \lambda_{y}\gamma\proj_{X^\bot} (q^k)
% 	\end{cases}
% 	\label{eq:progdec-contributions}
% \end{equation}
% where \(x^0 \in X\) and \(y^0 \in X^\bot\).
% In the standard progressive decoupling method the relaxation parameters $\lambda_{x}$ and $\lambda_{y}$ are chosen equal to one, while in Spingarn's method also $\gamma$ is fixed to one.

% Inspired by \cite{spingarn1983Partial}, we show that progressive decoupling+ can be viewed as a particular instance of the relaxed preconditioned proximal point algorithm (PPPA) applied to the \emph{partial inverse} of the operator $S$ (see \cref{lem:equivalence:PPPA-progdec}).
% As it will become clear in \cref{sec:progdec}, employing two distinct relaxation parameters allows us to more accurately account for the nonmonotonicity of the operator $S$.

% Our first contribution lies in extending the convergence results of \cite{evens2023convergence} for PPPA in the nonmonotone setting.
% In particular, we study local convergence of PPPA whenever the so-called oblique weak Minty condition condition holds locally. 
% By leveraging these new developments for PPPA, we show that (local) convergence of \ref{eq:progdec} can be established for linkage problems \eqref{prob:linkage-intro} even when $S$ is nonmonotone on both subspaces $X$ and $X^\bot$.
% Interestingly, our resulting theory encompasses and extends the results from \cite{rockafellar2019Progressive} for Spingarn's method of partial inverses and progressive decoupling in the elicitable monotone setting, allowing for more nonmonotonicity of the operator $S$ (see also \cref{rem:progdec:special-cases}).
% This additional degree of nonmonotonicity is quantified through the concept of \emph{semimonotonicity}, first introduced in \cite{evens2023convergence,evens2023convergenceCP}.

% First, we establish that progressive decoupling+ can be cast as a particular instance of the relaxed preconditioned proximal point algorithm (PPPA) applied to the \emph{partial inverse} of the operator $S$ (see \cref{lem:equivalence:PPPA-progdec}).
% Building upon the (global) convergence results from \cite{evens2023convergence} for relaxed PPPA in the nonmonotone setting, we establish the local convergence of relaxed PPPA for a class of nonmonotone operators that are defined through an oblique weak Minty condition.
% Applying this result, we show that convergence of \ref{eq:progdec} can be established for linkage problems \eqref{prob:linkage-intro} even when $S$ is nonmonotone on both subspaces $X$ and $X^\bot$. Interestingly, this convergence result also extends the class of problems solved by Spingarn's method of partial inverses and standard progressive decoupling.

In this work, we study a novel algorithm, progressive decoupling+, for solving linkage problems \eqref{prob:linkage-intro} in the nonmonotone setting.
It generalizes the standard progressive decoupling algorithm by incorporating two relaxation parameters, $\lambda_x$ and $\lambda_y$, which allow for greater flexibility in handling the (non)monotonicity of the operator $S$.
Specifically, given an initial guess \(x^0 \in X\) and \(y^0 \in X^\bot\), the iterates are as follows:
\begin{equation}
	\begin{cases}
		\displaystyle   
		q^k &\in J_{\gamma^{-1} S}(x^k + \gamma^{-1}y^k)\\
		x^{k+1}&= (1 - \lambda_{x})x^{k} + \lambda_{x}\proj_X (q^k)\\
		y^{k+1}&= y^{k} - \lambda_{y}\gamma\proj_{X^\bot} (q^k).
	\end{cases}
	\label{eq:progdec-contributions}
\end{equation}
Our main contributions can be summarized as follows.
\begin{enumerate}
	\item First, we establish a connection between progressive decoupling+ and the preconditioned proximal point algorithm (PPPA). Inspired by \cite{spingarn1983Partial}, we show in \cref{lem:equivalence:PPPA-progdec} that progressive decoupling+ can be interpreted as a relaxed variant of PPPA with matrix relaxation parameters, applied to the so-called \emph{partial inverse} of $S$ (see \cref{def:partial}).
	
	\item Our second contribution lies in extending the convergence results for PPPA from \cite{evens2023convergence} for nonmonotone problems which admit so-called oblique weak Minty solutions.
	This extension involves (i) generalizing the definition of weak Minty solutions to the local setting, only requiring the involved inequality to hold on a subset of the graph and (ii) allowing matrix relaxation parameters in the update rule, which is essential for linking it to our algorithm (see \Cref{lem:equivalence:PPPA-progdec}). 
	The localization of the graph is inspired by the local analysis for the proximal point algorithm in the maximally comonotone setting \cite{pennanen2002Local,iusem2003Inexact,combettes2004proximal}.

	\item 
	By leveraging these developments for PPPA, we establish the local convergence of progressive decoupling+ under the assumption that the operator
	\(
		(S - \mon \proj_{X^\bot})^{-1} - \com \proj_X
	\)
	is (locally) monotone for some \(\mon \in \R\) and \(\com \in \R\), a condition referred to as \((\mon \proj_{X^\bot}, \com \proj_X)\)-semimonotonicity of \(S\) \cite{evens2023convergence, evens2023convergenceCP, quan2024scaled}.
	This class of operators strictly encompasses both the elicitable monotone setting (retrieved for \(\com = 0\)) and the standard monotone setting (retrieved for \(\mon = \com = 0\)).

	The key device enabling this convergence result is summarized in \Cref{cor:partialinverse:semi-WMVI}, which establishes the equivalence between \((\mon \proj_{X^\bot}, \com \proj_X)\)-semimonotonicity of \(S\) and the existence of oblique weak Minty solutions for its partial inverse \(S^X\).
	Additionally, we demonstrate that our resulting conditions on the relaxation parameters \(\lambda_x\) and \(\lambda_y\) are tight through a simple linear example, and provide an example which is \((\mon \proj_{X^\bot}, \com \proj_X)\)-semimonotone but not elicitable monotone (see \cref{subsec:progdec:examples}).

	\item 
	Our algorithm recovers the standard progressive decoupling method for \(\mon \leq 0\), \(\lambda_x = 1\), and \(\lambda_y = 1 + \nicefrac{\mon}{\gamma}\), and reduces to Spingarn's method when \(\gamma = \lambda_x = \lambda_y = 1\). 
	By specializing to these two configurations, we show that our convergence theory both encompasses and extends existing convergence results for Spingarn's method of partial inverses and standard progressive decoupling, allowing for greater nonmonotonicity in the operator \(S\) (see also \cref{rem:progdec:special-cases}).

	\item
	To illustrate that the class of \((\mon\proj_{X^\bot}, \com \proj_X)\)\hyp{}semimonotone operators emerges quite naturally in practical applications, we provide several illustrative examples throughout the paper.
	Moreover, we provide calculus rules for
	determining whether a continuously differentiable function or mapping is $(\mon \proj_{X^\bot}, \com \proj_X)$-semimonotone
	in \cref{sec:linear}.
\end{enumerate}

==> TeX/Text/Preliminaries/preliminaries.tex <==

% \hl{Unused?}
% \begin{fact}\label{fact:partial-elicit} 
%     Let \(X\subseteq \R^n\) be a closed linear subspace, let \(A:\R^n\rightrightarrows\R^n\) be a set-valued operator.
%     Let $\theta \in [0, +\infty)$ and define $B = A + \theta \proj_{X^\bot}$ and the partial inverse of $B$ by $B^X$. Then, the following hold.
%     \begin{enumerate}
%         \item\label{it:fact:partial-elicit} Let $x, u \in X$ and $y, v \in X^\bot$. Then,
%         \((x+y, u+v) \in \gph A 
%         % \Leftrightarrow (x + y, u + v + \theta y) \in \gph B 
%         \Leftrightarrow (x + v + \theta y, u + y) \in \gph B^X\).
%         \item\label{it:fact:partial-elicit:zero} \(z \in \zer B^X 
%         % \Leftrightarrow (x + y, u + v + \theta y) \in \gph B 
%         \Leftrightarrow (\proj_X(z), \proj_{X^\bot}(z)) \in \gph A\).
%     \end{enumerate}
% \end{fact}


==> TeX/Text/Proofs/DRS/semi-Minty.tex <==
\begin{appendixproof}{prop:partialinverse:implications}
    \begin{proofitemize}
        \item \ref{it:partialinverse:implications:semi}: Let $(u, v) \in \gph S^X$ and recall that 
        $
          (x, y) = L_X(u, v)
            =     
          \big(\proj_X(u) + \proj_{X^\bot}(v), \proj_X(v) + \proj_{X^\bot}(u)\big)
            \in
          \gph S
        $
        and
        $
          (x^\star, y^\star) = L_X(u^\star, 0)
            =
          \big(\proj_X (u^\star), \proj_{X^\bot}(u^\star)\big)
            \in
          \gph S
        $.
        Therefore, owing to \Cref{it:spingarn:inner,it:spingarn:qindef} it holds that
        \begin{align*}
            \inner{v, u - u^\star} 
              {}={}
            \inner{y - y^\star, x - x^\star} 
            % \inner{\proj_X(u) + \proj_{X^\bot}(x) - \proj_{X^\bot}(x^\star), \proj_X(x) + \proj_{X^\bot}(u) - \proj_X(x^\star)}\\
              {}\geq{}
            \qindef{v}{V}
              % {}={}
            % \qindef{u}{\com \proj_{X}} + \qindef{u}{\mon \proj_{X^\bot}}
              {}={}&
            % \com\nrm{\proj_{X}(y)}^2 + \mon\nrm{\proj_{X^\bot}(x)}^2
            \qindef{y}{\com \proj_{X}} + \qindef{x}{\mon \proj_{X^\bot}}
              {}={}
            \qindef{y - y^\star}{\com \proj_{X}} + \qindef{x - x^\star}{\mon \proj_{X^\bot}},
        \end{align*}
        where the final equality holds since $x^\star \in X$ and $y^\star \in X^\bot$.
        \item \ref{it:partialinverse:implications:WMVI}: 
        Note that $\gph N_X = \set {(x_N,y_N)}[x_N \in X,\, y_N \in X^\bot]$.
        Therefore, 
        \(
          \big(\proj_X (u^\star), -\proj_{X^\bot}(u^\star)\big)
          \in
          \gph N_X
        \),
        so that by \cite[Prop. 6.9.2]{auslender2006asymptotic} it holds that
        \(
          \big(\proj_X (u^\star), \proj_{X^\bot}(u^\star)\big)
          \in
          \zer \Tpd
        \).
        Moreover, it holds for all $(x_N, y_N) \in \gph N_X$ and $(x_S, y_S) \in \gph S$ that
        \begin{align*}
            \inner*{
              \begin{bmatrix}
                y_N + y_S\\
                x_S - x_N
              \end{bmatrix}
              ,
              \begin{bmatrix}
                x_N - \proj_X (u^\star)\\
                y_S - \proj_{X^\bot}(u^\star)
              \end{bmatrix}
              }
                {}={}&
            \inner*{y_N + y_S, x_N - \proj_X (u^\star)} 
            + \inner*{x_S - x_N, y_S - \proj_{X^\bot}(u^\star)}\\
              {}={}&
            \inner*{y_N + \proj_{X^\bot}(u^\star), x_N - \proj_X (u^\star)} 
            + \inner*{x_S - \proj_X (u^\star), y_S - \proj_{X^\bot}(u^\star)}\\
              {}\geq{}&
            \qindef{x_S - \proj_X (u^\star)}{\mon \proj_{X^\bot}}
              +
            \qindef{y_S - \proj_{X^\bot}}{\com \proj_{X}}\\
              {}={}&
            \qindef{x_S - x_N}{\mon \proj_{X^\bot}}
              +
            \qindef{y_N + y_S}{\com \proj_{X}}
              ,
            % \geq 
            % \qindef{y_\A + L^\top y_\B}{\DRSRho_{\rm P}}
            % + \qindef{x_\B - L x_\A}{\DRSRho_{\rm D}},
            % \quad
            % \begin{cases}
            %     \forall (x^\star, y^\star) \in \pazocal{S}^\star,\\
            %     \forall (x_\A,y_\A) \in \gph \A,\\
            %     \forall (x_\B, y_\B) \in \gph B.
            % \end{cases}
            \numberthis\label{eq:WMI:primal-dual}
        \end{align*}
        where we used \cref{it:partialinverse:implications:semi} and monotonicity of $N_X$ \cite[Ex. 20.26]{bauschke2017Convex} to obtain the inequality and the fact that $x_N \in X$ and $y_N \in X^\bot$ in the final equality.
        Noting that
        \[
            \gph \Tpd = \set{\bigl((x_N, y_S),
            (y_N + y_S, 
            x_S - x_N)\bigr)}[(x_N, y_N) \in \gph N_X, (x_S, y_S) \in \gph S],
        \]
        the proof is completed.
    \end{proofitemize}
\end{appendixproof}

==> TeX/Text/Proofs/Examples/VonNeumann.tex <==
%!TEX root = ../../../Progdec-Minty.tex

\begin{appendixdetail}{ex:VonNeumann}
    We proceed by establishing three intermediate facts for the operators $F$ and $N_{\set{\tilde z \,\geq\, 0}}$. 
    % To start, we establish three identities for the set $C \coloneqq \Delta_2 \times \Delta_2$ and the operators $F$ and $N_C$. 
    First, recall that 
    \ifspringer
        $
            F(z)
                \coloneqq
            \left(%
                F_1(z), F_2(z), F_3(z), F_4(z)
            \right)
                {}={}
            \left(
                \nabla_x f(x,y), - \nabla_y f(x,y)
            \right)
        $, which is equal to 
        $
        \left(
            \tfrac{\inner{x, Sy} Ry - \inner{x, Ry} Sy}{\inner{x, Sy}^2},
            \tfrac{\inner{x, Ry} S^\top x - \inner{x, Sy} R^\top x}{\inner{x, Sy}^2}
        \right).
        $
    \else
        \[
            F(z)
                {}={}
            \left(%
                F_1(z), F_2(z), F_3(z), F_4(z)
            \right)
                {}={}
            \left(
                \nabla_x f(x,y), - \nabla_y f(x,y)
            \right)
                {}={}
            \left(
                \tfrac{\inner{x, Sy} Ry - \inner{x, Ry} Sy}{\inner{x, Sy}^2},
                \tfrac{\inner{x, Ry} S^\top x - \inner{x, Sy} R^\top x}{\inner{x, Sy}^2}
            \right).
        \]
    \fi
    Denoting the vector of all $1$s
    of dimension $n$ by $\mathbf{1}_n$, it holds that
    \begin{align*}
        N_{\set{z \,\geq\, 0}}(z)
        \begin{cases}
            \set{
                -\beta
            \,\middle|\,
            \beta \in \R_+^4,
            \inner{\beta, z} = 0}, &\qquad \text{if } z \geq 0,\\
            \emptyset, &\qquad \text{otherwise}.
        \end{cases}
        \numberthis\label{eq:VonNeumann:NC}
    \end{align*}
    We now proceed with the main argument.
    In \cite[Prop. 2(1)]{daskalakis2020independent}, it was shown that
    $
        z^\star =         
        % \begin{bsmallmatrix}
        %     0 & 1 & 0 & 1
        % \end{bsmallmatrix}^\top
        (0,1,0,1)
    $ is the unique Nash equilibrium of \eqref{eq:ex:neumann} (noting that 
    $
        f(x, y) - 2 =\nicefrac{
            \inner{x,         
            \begin{bsmallmatrix}
                -1 & \nicefrac{\varepsilon}{2}\\
                - \nicefrac{\varepsilon}{2} & 0
            \end{bsmallmatrix}y
        }}{{\inner{x, Sy}}}
    $).
    % Consequently, it follows from \cite[Prop. 2]{daskalakis2020independent} that $z^\star$ is the unique Nash equilibrium of \eqref{eq:ex:neumann}.
    This Nash equilibrium is a $\DRSrho_\varepsilon$\hyp{}weak Minty solution of $T$ provided that
    \(
        \DRSrho_\varepsilon
            {}={}
        \inf_{z \in C} \varrho_\varepsilon(z)
    \)
    where
    \(
        \varrho_\varepsilon(z)
            {}={}
        \inf_{v \in N_C(z)}
        \nicefrac{
            \inner*{F(z) + v,z-z^\star}
        }
        {
            \nrm{F(z) + v}^2
        }
    \).
    From now onwards, we tacitly assume that $z \in C$. Then, owing to \eqref{eq:VonNeumann:NC}, it holds that
    \begin{align*}
        \varrho_\varepsilon(z)
            {}={}
        \inf\set{
        \tfrac{%
            \inner*{% 
                F(z),
                z - z^\star
            } 
                -
            \inner*{                   
                \beta,
                z - z^\star
            } 
        }
        {\nrm{
            F(z)
                -
            \beta
        }^2
        }%
        }
        [\beta \in \R_+^4, 
        \;\inner{
            \beta,
            z
        } 
        = 0
        ].
    \end{align*}
    Owing to the parametrization from \eqref{eq:VonNeumann:parametrization} and the fact that    
    $
        z^\star =
            (0,1,0,1)
    $,
    it holds that
    \(
        \inner*{                   
                \alpha \otimes 
                \mathbf{1}_2,
                z - z^\star
            }
            {}={}
        0
    \) 
    and
    $\inner{\beta, z^\star} = \beta_2 + \beta_4$, so that
    \begin{align*}
        \varrho_\varepsilon(z)
            {}={}& 
        \inf\set{
            \tfrac{
                \inner*{ 
                    F(z),
                    z - z^\star
                } 
                    +
                \beta_2
                    +
                \beta_4
            }
            {\nrm{
                F(z)
                    -
                \beta
            }^2
            }
        }
        [\beta \in \R_+^4, 
        \,\inner{
            \beta,
            z
        } 
        = 0
        ].
    \end{align*}
    Note that by construction the sign of $\varrho_\varepsilon(z)$ is equal to the sign of 
    $            
        \inner*{ 
            F(z),
            z - z^\star
        }
    $:
    if
    \(\inner*{ 
        F(z),
        z - z^\star
    }\)
    is positive, this is obvious since \(\beta_i \geq 0\); if it is negative, then this can be seen by taking the candidate solution $\beta_2 = \beta_4 = 0$.
    Therefore, it follows from \eqref{eq:VonNeumann:F} that $\varrho_\varepsilon(z) < 0$
    % By \eqref{eq:VonNeumann:F} it holds that
    % \(
    %     \inner*{ 
    %         F(z),
    %         z - z^\star
    %     }
    %         <
    %     0
    % \)
    if and only if
    \(
        \varepsilon(s + t)
            -
        st(\varepsilon + s)
            <
        0
    \), i.e., if and only if $z$ lies in the nonempty set
    \[
        D
            \coloneqq
        \set{(s, 1-s, t, 1-t)}
        [{s \in (\hspace{-2pt}\sqrt{\varepsilon}, 1],\, t \in (\bar{t}(s), 1]}],
            \quad\text{where}\quad
        \bar{t}(s)
            {}\coloneqq{}
        \tfrac{\varepsilon s}{s(\varepsilon + s)-\varepsilon}.
    \]
    Therefore, 
    \(
        \DRSrho_\varepsilon
            {}={}
        \inf_{z \in C} \varrho_\varepsilon(z)
            {}={}
        \inf_{z \in D} \varrho_\varepsilon(z).
    \)
    Let $z \in D \subset C$. Then, by construction $\varrho_\varepsilon(z)$ is negative, which implies that \(\varrho_\varepsilon(z)\) is minimized for \(\alpha\) minimizing the denominator. Using that
    \[
        \argmin_{\alpha \in \R^2} \;
        \nrm{
            F(z)
                +                         
            \alpha \otimes 
            \mathbf{1}_2
            -
            \beta
        }^2
            {}={}
        \left(
            \tfrac12(F_1(z) - F_2(z) - \beta_1 + \beta_2), 
            \tfrac12(F_3(z) - F_4(z) - \beta_3 + \beta_4)\right),
    \]
    this implies that
    \begin{align*}
        \varrho_\varepsilon(z)
            {}={}& 
        \inf\set{\tfrac{
            2\inner*{ 
                F(z),
                z - z^\star
            } 
                +
            2\beta_2
                +
            2\beta_4
        }
        {
            \bigl(
                F_1(z) - \beta_1 - F_2(z) + \beta_2
            \bigr)^2
                +
            \bigl(
                F_3(z) - \beta_3 - F_4(z) + \beta_4
            \bigr)^2
        }
        }[
            \beta \in \R_+^4,
            \,
            \inner{
                \beta,
                z
                } 
            = 0
        ].
    \end{align*}
    Plugging in the parametrization for $z$ from \eqref{eq:VonNeumann:parametrization}, using \eqref{eq:VonNeumann:F} and introducing $\bar{\beta} \coloneqq \nicefrac12(2 - s)^2\beta$, it follows that
    \begin{align*}
        \varrho_{\varepsilon}(s,t)
            {}={}
        \inf\set{
        \tfrac{
            4(2 - s)^2
            \bigl(
                \varepsilon(s + t)
                    -
                st(\varepsilon + s)
                    +
                \bar{\beta}_2
                    +
                \bar{\beta}_4
            \bigr)
        }
        {
            \bigl(
                2\varepsilon - t(4 + \varepsilon)
                -
                2\bar{\beta}_1
                + 
                2\bar{\beta}_2
            \bigr)^2
                +
            \bigl(
                (\varepsilon + 2s)(2 - s)
                -
                2\bar{\beta}_3
                +
                2\bar{\beta}_4
            \bigr)^2
        }
        }[
            \bar{\beta} \in \R_+^4,\,
            \inner{
            \bar{\beta},
            (s, 1-s, t, 1-t)
            } 
        = 0
        ],       
    \end{align*}
    % \begin{figure}
    %     \centering
    %     \includetikz{Examples/VonNeumann/lower-bound}
    %     \caption{
    %         \begin{new}
    %             Comparison between the optimal weak Minty constant $\DRSrho_\varepsilon$ and its lower bound $\tfrac{\varepsilon - 1}{4}$ for \cref{ex:VonNeumann}.
    %         \end{new}
    %         }
    %     \label{fig:VonNeumann:rho}
    % \end{figure}%
    We claim that $\bar \beta = 0$ at the infimum for any $s \in (\hspace{-2pt}\sqrt{\varepsilon}, 1]$ and $t \in (\bar{t}(s), 1]$.
    For $\bar \beta_1$ and $\bar \beta_3$, this follows from the equality constraint and the fact that $s$ and $t$ are strictly positive, so that
    \begin{align*}
        \varrho_{\varepsilon}(s,t)
            {}={}
        \inf\set{
        \tfrac{
            4(2 - s)^2
            \bigl(
                \varepsilon(s + t)
                    -
                st(\varepsilon + s)
                    +
                \bar{\beta}_2
                    +
                \bar{\beta}_4
            \bigr)
        }
        {
            \bigl(
                2\varepsilon - t(4 + \varepsilon)
                + 
                2\bar{\beta}_2
            \bigr)^2
                +
            \bigl(
                (\varepsilon + 2s)(2 - s)
                +
                2\bar{\beta}_4
            \bigr)^2
        }
        }[
            (\bar{\beta}_2, \bar{\beta}_4) \in \R_+^2,\,
            \inner{
                (\bar{\beta}_2, \bar{\beta}_4),
                (1-s, 1-t)
                } 
            = 0
        ].
    \end{align*}
    If $s \in (\hspace{-2pt}\sqrt{\varepsilon}, 1)$ and $t \in (\bar{t}(s), 1)$, the claim for $\bar \beta_2$ and $\bar \beta_4$ also follows from the equality constraint. Otherwise, consider the following cases.
    \begin{proofitemize}
        \item If $s = 1$ and $t \in (\bar{t}(1), 1) = (\varepsilon, 1)$, then $\bar{\beta}_4 = 0$ due to the equality constraint and
        \begin{align*}
            \varrho_{\varepsilon}(1,t)
                {}={}
            \inf_{
                \bar{\beta}_2 \in \R_+
            } \; 
            \tfrac{
                4
                (
                    \varepsilon
                        -
                    t
                        +
                    \bar{\beta}_2
                )
            }
            {
                \bigl(
                    2\varepsilon - t(4 + \varepsilon)
                    + 
                    2\bar{\beta}_2
                \bigr)^2
                    +
                (
                    \varepsilon + 2
                )^2
            }
                {}={}
            \inf_{
                \bar{\beta}_2 \in [0, t - \varepsilon)
            } \; 
            \tfrac{
                4
                (
                    \varepsilon
                        -
                    t
                        +
                    \bar{\beta}_2
                )
            }
            {
                \bigl(
                    2\varepsilon - t(4 + \varepsilon)
                    + 
                    2\bar{\beta}_2
                \bigr)^2
                    +
                (
                    \varepsilon + 2
                )^2
            }.
        \end{align*}
        Since this function is monotonically increasing for $\bar{\beta}_2 \in [0, t - \varepsilon)$, the infimum is attained for $\bar{\beta}_2 = 0$.
        \item If $s \in (\hspace{-2pt}\sqrt{\varepsilon}, 1)$ and $t = 1$, then $\bar{\beta}_2 = 0$ due to the equality constraint and
        \begin{align*}
            \varrho_{\varepsilon}(s,1)
                {}={}
            \inf_{
                \bar{\beta}_4 \in \R_+
            } \; 
            \tfrac{
                4(2 - s)^2
                (
                    \varepsilon
                        -
                    s^2
                        +
                    \bar{\beta}_4
                )
            }
            {
                (
                    \varepsilon - 4
                )^2
                    +
                \bigl(
                    (\varepsilon + 2s)(2 - s)
                    +
                    2\bar{\beta}_4
                \bigr)^2
            }
                {}={}
            \inf_{
                \bar{\beta}_4 \in [0, s^2 - \varepsilon)
            } \; 
            \tfrac{
                4(2 - s)^2
                (
                    \varepsilon
                        -
                    s^2
                        +
                    \bar{\beta}_4
                )
            }
            {
                (
                    \varepsilon - 4
                )^2
                    +
                \bigl(
                    (\varepsilon + 2s)(2 - s)
                    +
                    2\bar{\beta}_4
                \bigr)^2
            }.
        \end{align*}
        Since this function is monotonically increasing for $\bar{\beta}_4 \in [0, s^2 - \varepsilon)$, the infimum is attained for $\bar{\beta}_4 = 0$.
        \item If $s = 1$ and $t = 1$, then
        \ifspringer
            \(
                \varrho_{\varepsilon}(1,1)
                    {}={}
                \inf_{
                    (\bar{\beta}_2, \bar{\beta}_4) \in \R_+^2
                } \; 
                \smash{
                \tfrac{
                    4
                    (
                        \varepsilon
                            -
                        1
                            +
                        \bar{\beta}_2
                            +
                        \bar{\beta}_4
                    )
                }
                {
                    (
                        \varepsilon - 4
                        + 
                        2\bar{\beta}_2
                    )^2
                        +
                    (
                        \varepsilon + 2
                        +
                        2\bar{\beta}_4
                    )^2
                }}
            \),
        \else
            \begin{align*}
                \varrho_{\varepsilon}(1,1)
                    {}={}
                \inf_{
                    (\bar{\beta}_2, \bar{\beta}_4) \in \R_+^2
                } \; 
                \tfrac{
                    4
                    (
                        \varepsilon
                            -
                        1
                            +
                        \bar{\beta}_2
                            +
                        \bar{\beta}_4
                    )
                }
                {
                    (
                        \varepsilon - 4
                        + 
                        2\bar{\beta}_2
                    )^2
                        +
                    (
                        \varepsilon + 2
                        +
                        2\bar{\beta}_4
                    )^2
                },
            \end{align*}
        \fi
        of which the global minimum is attained for $\bar{\beta}_2 = \bar{\beta}_4 = 0$.
    \end{proofitemize}
    Having established that $\bar \beta = 0$ at the infimum, it follows that
    \begin{align*}
        \DRSrho_\varepsilon
            {}={}& 
        \inf\set{
            \,\varrho_\varepsilon(s, t)
        }[
            {
            s \in (\sqrt{\varepsilon}, 1],\,
            t \in \left(
                    \tfrac{\varepsilon s}{s(\varepsilon + s)-\varepsilon}, 1
                \right]
            }
        ],
            \quad\text{where}\quad
        \varrho_\varepsilon(s, t)
            =
        \tfrac{
            4(2 - s)^2
            \bigl(
                \varepsilon(s + t) - st(\varepsilon + s)
            \bigr)
        }
        {
            \bigl(
                2\varepsilon - t(4 + \varepsilon)
            \bigr)^2
                +
            (\varepsilon + 2s)^2(2 - s)^2
        }.
    \end{align*}
    Finally, the lower bound $\tfrac{\varepsilon - 1}{4} \leq \DRSrho_\varepsilon$ is obtained by solving this parametric optimization problem numerically (see also \Cref{fig:VonNeumann:rho}).
\end{appendixdetail}

==> TeX/Text/Proofs/pppa-relax.tex <==

\begin{appendixproof}{thm:pppa}
    If $z^k \in \mathcal{D}_{z^k, \bar z^k}$ for some $k \in \N$ then by \Cref{half:xbar} the algorithm has reached a point $\bar{z}^k \in \zer T$ in a finite number of iterations. Therefore, we consider the case when $z^k \notin \mathcal{D}_{z^k, \bar z^k}$ in the remainder of the proof.
    \begin{proofitemize}
        \item \ref{it:pppa:v}:
        Owing to \Cref{half:update} it holds for any $z^\star\in \pazocal{S}^\star$ that
        \begin{align}\label{eq:iFejer}
            \|z^{k+1}-z^\star\|_{\M \Lambda^{-1}}^2
                {}\leq{}
            \|z^k-z^\star\|_{\M \Lambda^{-1}}^2-(\nicefrac2\lambda-1)\|z^k-\bar{z}^k\|_{\M \Lambda}^2,
        \end{align}
        establishing that $(z^k)_{k\in\N}$ is Fej\'er monotone with respect to $\pazocal{S}^\star$ \cite[Def. 5.1]{bauschke2017Convex}.
        The claimed convergence of $\seq{z^k - \bar z^k}$ and its corresponding rate are obtained by telescoping \eqref{eq:iFejer}.
        % ,
        % it follows that 
        % \(\sum_{k = 0}^\infty \|z^k - \bar z^k\|^2_{\M H} < +\infty\), which implies that 
        % $\seq{z^k - \bar z^k}$ converges to zero.
        % The claimed rate follows by telescoping \eqref{eq:iFejer}.

        \item \ref{it:pppa:bounded}:
        From the update rule~\eqref{eq:PPPA-intro}, it directly follows that
        \(
            \bar v^k \coloneqq \M(z^k - \bar{z}^k) \in T \bar{z}^k    
        \)
        for all $k$. It remains to show that $\seq{\bar v^k}$ converges to zero.
        The convergence of $(\bar{v}^k)_{k\in N}$ to zero is established by noting that
        \begin{align*}
            \|\bar{v}^k\|^2
                {}={}
            \|\M(z^k-\bar{z}^k)\|^2
                {}\leq{}
            \|\M^{\nicefrac12}\Lambda^{\nicefrac{-1}2}\|^2\, \|\Lambda^{\nicefrac12}\M^{\nicefrac12}(z^k-\bar{z}^k)\|^2
                {}={}
            \nrm{\M \Lambda^{-1}}\, \|z^k-\bar{z}^k\|^2_{\M \Lambda}.
            \numberthis\label{eq:vw}
        \end{align*}
        Since \((\bar v^k)_{k\in\N}\) converges to zero and $\bar{v}^k\in T\bar{z}^k$, it follows from outer semicontinuity of $T$ (due to \Cref{ass:PPPA:0}) that any limit point of $(\bar{z}^k)_{k\in\N}$ belongs to $\zer T$.
        Moreover, it follows from \eqref{eq:iFejer} that \(\seq{\|z^k - z^\star\|_{\M \Lambda^{-1}}}\) converges, and in particular that $(z^k)_{k\in\N}$ is bounded. In turn, using 
        that $\|z^k - \bar z^k\|_{\M \Lambda} \to 0$
        and the triangle inequality 
        \(
            \|\bar{z}^k\|_{\M \Lambda} \leq \|\bar{z}^k-z^k\|_{\M \Lambda}+\|z^k\|_{\M \Lambda},
        \)
        it follows that \(\seq{\bar{z}^k}\) is bounded and thus that it has at least one limit point.
        Take a subsequence $(\bar{z}^k)_{k\in K}$ converging to some limit point $z^\infty \in \zer T$. Since $(\bar{z}^k-z^k)_{k\in\N}$ converges to zero
        as shown in \Cref{it:pppa:v},
        we have that $(z^k)_{k\in K}$ also converges to the same limit point $z^\infty$.

        \item \ref{it:pppa:full}:
        If $\pazocal{S}^\star=\zer T$,
        then the convergence of $(z^k)_{k\in\N}$
        to some element of $\zer T$ follows by~\cite[Thm. 5.5]{bauschke2017Convex}, and $(\bar z^k)_{k\in\N}$ converges to the same point owing to \Cref{it:pppa:v}.
        \qedhere
    \end{proofitemize}
\end{appendixproof}

==> TeX/Text/deprecated/ProbForm.tex <==
%!TEX root = ../../../ProgDec-Minty.tex

Departing from the classical monotone setting, convergence of relaxed \ref{eq:PPPA-intro} was established in \cite{evens2023convergence} for a class of nonmonotone operators that admit a set of \emph{oblique weak Minty solutions} (see \cref{def:SWMVI}). This result will serve as our primary tool for establishing convergence of \ref{eq:progdec} in the nonmonotone setting, which is why we will reiterate it here.
In particular, their analysis involves the following assumptions, where we assume here positive definiteness of $\M$ for simplicity.
\begin{assumption} \label{ass:PPPA}
    The operator \(T: \R^{n} \rightrightarrows \R^n\), preconditioner \(\M \in \sym{n}\) and relaxation matrix \(\Lambda \in \sym{n}\) in \eqref{eq:PPPA-intro} satisfy the following properties. 
    \begin{enumeratass}
        \item \label{ass:PPPA:1} 
        There exists a nonempty set \(\pazocal{S}^\star\subseteq \zer T\) and a symmetric, possibly indefinite matrix \(V \in \sym{n}\) such that \(T\) has $\DRSRho$\hyp{}oblique weak Minty solutions at \(\pazocal{S}^\star\).
        \item \label{ass:PPPA:0} \(T\) is outer semicontinuous.
        \item \label{ass:PPPA:0.5} The preconditioned resolvent \((\M + T)^{-1}\circ\M\) has full domain.
        \item \label{ass:PPPA:2} \(\M\) and \(\Lambda\) are positive definite matrices satisfying \(\Lambda \M = \M \Lambda\). Moreover, there exists a $\lambda \in (0,2)$ such that
        \begin{equation}\label{eq:PPPA:eigcond}
            \lambda(\I + \M^{\nicefrac12} \DRSRho \M^{\nicefrac12}) \succeq \Lambda.
            % \quad\text{and}\quad \Lambda \M = \M \Lambda.
        \end{equation}
    \end{enumeratass}
\end{assumption}
In contrast to the convergence analysis techniques relying on firm nonexpansiveness of the resolvent mapping, the analysis of \cite{evens2023convergence} relies on a projective interpretation of the preconditioned proximal point algorithm, which dates back to \cite{solodov1996Modified,solodov1999hybrid,konnov1997Class}.
Most notably, it was demonstrated in \cite[Lem. 2.2]{evens2023convergence} that the update rule for the (shadow) sequence generated by \ref{eq:PPPA-intro} can be interpreted as a relaxed projection onto a certain halfspace, and that if any iterate belongs to this halfspace, which contains the set of projected oblique weak Minty solutions \(\projQ\pazocal{S}^\star\), this implies its optimality.
Based on this insight, the following convergence result for \ref{eq:PPPA-intro} was established.
% Owing to this projective interpretation and non-expansiveness of the projection operator, the following convergence result for the preconditioned proximal point algorithm was obtained.

\begin{theorem}[convergence of \ref{eq:PPPA-intro}]\label{thm:pppa}
    Suppose that \cref{ass:PPPA} holds, and consider a sequence $\seq{z^k, \bar z^k}$ generated by \ref{eq:PPPA-intro} starting from $z^0 \in \R^n$.
    Then, either a point $\bar z^k \in \zer T$ is reached in a finite number of iterations or 
    the following hold for the sequence $\seq{z^k, \bar z^k}$.
    \begin{enumerate}
        \item\label{it:pppa:v} $\M(z^k-\bar{z}^k)\in T\bar{z}^k$ for all \(k\) and $(z^k-\bar{z}^k)_{k\in \N}$ converges to zero with rate
        \begin{align*}
            \min_{k=0,1,\ldots,N} 
            \qindef{z^k - \bar z^k}{\M \Lambda^{-1}}
                {}\leq{}
            \frac1{(N+1)(\nicefrac{2}{\lambda} - 1)}
            \qindef{z^0-z^\star}{\M \Lambda^{-1}},
            \qquad\text{for all $z^\star\in\pazocal{S}^\star$}.
        \end{align*}
        \item\label{it:pppa:bounded} The sequences $(z^k)_{k\in\N}$, $(\bar{z}^k)_{k\in\N}$ are bounded and their limit points belong to $N \cap \zer T$.
        \item\label{it:pppa:full} 
        If in \cref{ass:PPPA:1} the set
        $ 
            \pazocal{S}^\star
        $
        is equal to
        $ 
            \zer T
        $, then the sequences
        $
            \seq{z^k}
        $,
        $
            \seq{\bar z^k}
        $
        converge
        to some element of $\zer T$.
    \end{enumerate}
    \begin{proof}
        See \Cref{proof:thm:pppa}.
    \end{proof}
\end{theorem}

%!TEX root = ../../../../DRS-Minty.tex

\begin{proposition}[resolvent of a comonotone operator]\label{prop:comon:fulldom}
    Let $T: \R^n \rightrightarrows \R^n$ be a $\DRSRho$\hyp{}comonotone operator and suppose that \(\M \succ 0\) is selected according to \Cref{ass:PPPA:2}.
    Then, the preconditioned resolvent \(\PRES\) is Lipschitz continuous with modulus
    \[
        L(\M) = \tfrac{\nrm{\M + \M\DRSRho\M} + \sqrt{\nrm{\M + \M\DRSRho\M}^2 - 4\lambda_{\rm min}(\M + \M\DRSRho\M)\lambda_{\rm min}(\M\DRSRho\M)}}{2\lambda_{\rm min}(\M + \M\DRSRho\M)}.
    \]
    \begin{proof}
        Take $(u,v), (\other{u}, \other{v}) \in \gph (\M + T)^{-1}\M$. By comonotonicity of \(T\) and using the fact that  
        \(
            \M(u-v) \in Tv,
        \) 
        \(
            \M(\other{u}-\other{v}) \in T\other{v}
        \),
        we have 
        \begin{align*}
            \qindef{(u-v)-(\other{u}-\other{v})}{\M\DRSRho\M}
            \leq
            \inner{\M \Bigl((u-v)-(\other{u}-\other{v})\Bigr), v-\other{v}}.
        \end{align*}
        Expanding the last term of the left-hand side and rearranging, we get
        \begin{align*}
            \qindef{u - \other{u}}{\M\DRSRho\M}
            +
            \qindef{v - \other{v}}{\M + \M\DRSRho\M}
                {}\leq{}&
            \inner{(\M + 2\M\DRSRho\M) (u-\other{u}), v-\other{v}},
            %     {}\leq{}&
            % \nrm{\M + 2\M\DRSRho\M}\nrm{u-\other{u}}\nrm{v-\other{v}}.
        \end{align*}
        which implies that
        \begin{align*}
            \lambda_{\rm min}(\M \DRSRho \M)\nrm{u - \other{u}}^2
            +
            \lambda_{\rm min}(\M + \M\DRSRho\M)\nrm{v - \other{v}}^2
                {}\leq{}&
            \nrm{\M + 2\M\DRSRho\M}\nrm{u-\other{u}}\nrm{v-\other{v}}
        \end{align*}
        If $\M \succ 0$, it holds that 
        \(\M + \M \DRSRho \M \succ 0\)
        by \Cref{ass:PPPA:2}.
        Hence, if \(u=\other{u}\) then necessarily \(v=\other{v}\), and the Lipschitz inequality holds trivially. 
        Otherwise, divide both sides by \(\|u-\other{u}\|^2\) to obtain 
        \begin{equation*}
                \lambda_{\rm min}(\M + \M\DRSRho\M)\omega^2
                    - 
                \nrm{\M + 2\M\DRSRho\M} \omega 
                    +
                \lambda_{\rm min}(\M \DRSRho \M)
                    \leq 0,
        \end{equation*}
        where     
        \(
            \omega \coloneqq \tfrac{\nrm{v-\other{v}}}{\nrm{u-\other{u}}}    
        \). 
        Solving this quadratic inequality for $\omega$ yields the claimed Lipschitz modulus.
    \end{proof}
\end{proposition}

% \input{TeX/Text/PPA/MetricSubreg.tex}

==> TeX/Text/deprecated/curvature.tex <==
In what follows, we present various function classes of which the (limiting) subdifferentials belong to the class of semimonotone operators.

\begin{proposition}[monotone versus nonexpansive mappings]\label{prop:mon-nonexp}
    Let $Y \subseteq \R^n$ be a closed, linear subspace. Consider an operator $T : \R^n \rightrightarrows \R^n$ and define $S \coloneqq \proj_Y - 2\id \circ (T + \proj_Y)^{-1}$.
    % , so that
    % \[
    %     (T + \proj_Y)^{-1} = \tfrac12(\proj_Y - S)
    % \]
    Then, $T$ is monotone on $Y \times Y$ if and only if $S$ is nonexpansive on $Y \times Y$ and $T$ is strictly monotone on $Y \times Y$ if and only if $S$ is contractive on $Y \times Y$.
    \begin{proof}
        Consider the linear operator $J : \R^n \times \R^n \rightarrow \R^n \times \R^n$ with $J(x, y) = (y + \proj_Y x, \proj_Y y + \proj_Y x - 2x)$.
        Then, it holds that
        \begin{align*}
            J(\gph T) 
                {}={}&
            \set{(y + \proj_Y x, \proj_Y y + \proj_Y x - 2x)}[(x,y) \in \gph T]\\
                {}={}&
            \set{(y, \proj_Y y - 2x)}[(x,y) \in \gph (T + \proj_Y)]\\
                {}={}&
            \set{(x, \proj_Y x - 2y)}[(x,y) \in \gph (T + \proj_Y)^{-1}]\\
                {}={}&
            \gph \bigl(\proj_Y - 2\id \circ (T + \proj_Y)^{-1}\bigr) = \gph S.
        \end{align*}
        Let $x, y, \other{x}, \other{y} \in \R^n$ and define $(z, w) = J(x, v)$ and $(\other{z}, \other{w}) = J(\other{x}, \other{y})$. Then,
        \begin{align*}
            \nrm{z-\other{z}}^2 - \nrm{w - \other{w}}^2
                {}={}&
            \inner{(z-\other{z})+(w-\other{w}),(z-\other{z})-(w-\other{w})}\\
                {}={}&
            \inner{(z+w)-(\other{z}+\other{w}),(z-w)-(\other{z}-\other{w})}.
        \end{align*}
        Since 
        $
            z+w = 
            2y - \proj_{Y^\perp}(y) - 2\proj_{Y^\perp}(x)
            % (\id + \proj_Y)y - 2(\id-\proj_Y)x
        $
        and
        $
            z-w = 2x + \proj_{Y^\perp}(y)
        $, it follows that
        \begin{align*}
            \nrm{z-\other{z}}^2 - \nrm{w - \other{w}}^2
                {}={}&
            \inner{2(y-\other{y}) - \proj_{Y^\perp}(y - \other{y}) - 2\proj_{Y^\perp}(x-\other{x}),2(x-\other{x}) + \proj_{Y^\perp}(y-\other{y})}\\
                {}={}&
            4\inner{y-\other{y}, x-\other{x}}
                -
            4\nrm{\proj_{Y^\perp}(x-\other{x})}^2
                -
            4\inner{y-\other{y}, \proj_{Y^\perp}(x-\other{x})}
                +
            \nrm{\proj_{Y^\perp}(y-\other{y})}^2.
        \end{align*}
        Note that $x, y, \other{x}, \other{y} \in Y$ if and only if $z, \other{z}, w, \other{w} \in Y$, in which case
        \begin{align*}
            \nrm{z-\other{z}}^2 \geq \nrm{w - \other{w}}^2
                \quad{}\Longleftrightarrow{}\quad
            \inner{y-\other{y},x-\other{x}} \geq 0,
        \end{align*}
        completing the proof.
    \end{proof}
\end{proposition}

\begin{lemma}[dualization of elicitable convexity]\label{lem:elic}
    Let $\sigma \in \R$ and let $Y \subseteq \R^n$ be a closed, linear subspace. Consider a proper lsc function $f : \R^n \rightarrow \R$. Then, the following are equivalent.
    \begin{enumerate}
        \item \label{it:lem:elic:1} $f - \tfrac{\sigma}{2}\| \proj_Y \cdot\,\|^2$ is convex.
        \item \label{it:lem:elic:2} $\partial f$ is $(\sigma \proj_Y, 0)$-semimonotone.
    \end{enumerate}
    \begin{proof}
        Follows by \cite[Thm. 12.17]{rockafellar2009Variational}.
    \end{proof}
\end{lemma}

\begin{lemma}[strong elicitable convexity and monotonicity]\label{lem:dual:elic}
    Let $\sigma > 0$ and let $Y \subseteq \R^n$ be a closed, linear subspace. Consider a proper lsc convex function $f : \R^n \rightarrow \R$. Then, the following are equivalent.
    \begin{enumerate}
        \item \label{it:lem:dual:elic:1} $g \coloneqq f^* - \tfrac{\sigma}{2}\| \proj_Y \cdot\,\|^2$ is proper lsc convex.
        \item \label{it:lem:dual:elic:1.5} $\partial g$ is maximally monotone.
        \item \label{it:lem:dual:elic:2} $f(x) = \inf_{w} \left\{g^*(x-w) + \tfrac{1}{2\sigma} \| w \|^2 + \delta_{\{0\}}(\proj_{Y^\perp}w)\right\}$.
        \item \label{it:lem:dual:elic:3} $\partial f^*$ is $(\sigma \proj_Y, 0)$-semimonotone.
        \item \label{it:lem:dual:elic:4} $\partial f$ is $(0, \sigma \proj_Y)$-semimonotone.
    \end{enumerate}
    Moreover, under these conditions $\partial f$ is Lipschitz continuous on $Y \times Y$ with constant $\tfrac{1}{\sigma}$, i.e.
    \begin{align*}
        \inner{y - \other{y}, x-\other{x}} \leq \tfrac{1}{\sigma}\nrm{x-\other{x}},
        \qquad
        \forall (x, y), (\other{x}, \other{y}) \in \gph \partial f \cap (Y \times Y).
    \end{align*}
    \begin{proof}
        Equivalence between \ref{it:lem:dual:elic:1} and \ref{it:lem:dual:elic:1.5} holds by \cite[Thm. 12.17]{rockafellar2009Variational}.
        Let $h(x) \coloneqq \tfrac{\sigma}{2}\| \proj_Y x\,\|^2$.
        Equivalence between \ref{it:lem:dual:elic:1} and \ref{it:lem:dual:elic:2} follows directly from \cite[Thm. 11.23(a)]{rockafellar2009Variational}, using that $h^*(v) = \tfrac{1}{2\sigma} \| v \|^2 + \delta_{\{0\}}(\proj_{Y^\perp}v)$. 
        Equivalence between \ref{it:lem:dual:elic:1} and \ref{it:lem:dual:elic:3} follows from \cref{lem:elic}. By convexity of $f$, it holds that $\partial f^* = (\partial f)^{-1}$, which by definition of semimonotonicity shows the equivalence with \ref{it:lem:dual:elic:4}.

        Finally if \ref{it:lem:dual:elic:1.5} holds then $\tfrac1\sigma\partial g$ is monotone (on $Y \times Y$) and it follows by \Cref{prop:mon-nonexp} that there exists an operator $S$ such that
        $
            \partial f = \tfrac1\sigma(\tfrac12(\proj_Y - S)) \eqqcolon \tfrac1\sigma \tilde S
        $
        and that $S$ is nonexpansive on $Y \times Y$.
        By \cite[Prop. 12.10(b)]{rockafellar2009Variational}, this implies that $\tilde S \coloneqq \tfrac12\id \circ (\proj_Y - S)$ is also nonexpansive on $Y \times Y$, and thus that 
        $
            \partial f
        $
        is Lipschitz continuous on $Y \times Y$ with constant $\tfrac1\sigma$, completing the proof.
    \end{proof}
\end{lemma}

\begin{definition}[upper and lower curvature]
    Let \(\Sigma, L \in \sym{n}\). Consider a proper lsc function \(f:\R^n \to \Rinf\). Then, 
    \begin{enumerate}
        \item (lower curvature) \(f\) is said to have lower curvature with modulus \(\Sigma\)
        (denoted by \(f \in \mathcal F_{\Sigma}(\R^n)\))
        if  
        \(
            \varphi_{\Sigma} \coloneqq f - \tfrac12\qindef{\cdot}{\Sigma}
        \) is convex. %, where \(\sigma\in \R\). 
        \item (upper curvature) \(f\) is said to have upper curvature with modulus \(L\)
        (denoted by \(f \in \mathcal F^{L}(\R^n)\))
        if  
        \(f\) is finite-valued and
        \(
            \varphi^{L} \coloneqq \tfrac{1}2\qindef{\cdot}{L} - f
        \) is convex. %, where \(\ell\in \R\).
    \end{enumerate}
    A function with both lower curvature $\Sigma$ and upper curvature $L$ is denoted by \(\mathcal F_{\Sigma}^{L}(\R^n)\). 
\end{definition}
 
 
\begin{proposition}[functions with upper and lower curvature]\label{prop:curvature}
    Let \(\sigma, \ell \in \R\) and let $Y \subseteq \R^n$ be a closed, linear subspace. Consider a proper lsc function \(f:\R^n \to \Rinf\). 
    % Consider a proper lsc function \(f:\R^n \to \Rinf\). 
    % If \(f\in \mathcal F_{\sigma, X}^{\ell, Y}(\R^n)\), then, ...
    Then, the following hold.
    \begin{enumerate}
        \item \label{prop:hypo:cvx} If \(f \in \mathcal F_{\sigma\proj_Y}(\R^n)\), then $\partial f$ is $(\sigma\proj_Y, 0)$-semimonotone.
        \item \label{prop:hypo:ccv} If \(f\) is continuous and \(f \in \mathcal F^{\ell\proj_Y}(\R^n)\) with $\ell < 0$, then $\partial f$ is $(0, \tfrac1\ell\proj_Y)$-semimonotone on $Y \times Y$.
    \end{enumerate}
    \begin{proof}
        \begin{proofitemize}
            \item \ref{prop:hypo:cvx}: Follows by definition.
            \item \ref{prop:hypo:ccv}: Note that $-f - \tfrac{(-\ell)}{2}\nrm{\proj_Y \cdot\,}^2$ is convex, which owing to \Cref{lem:dual:elic} implies that $\partial (-f)^*$ is Lipschitz continuous on $Y \times Y$ with constant $-\tfrac{1}{\ell}$, i.e.
            \begin{align*}
                \inner{y - \other{y}, x-\other{x}} \leq -\tfrac{1}{\ell}\nrm{x-\other{x}},
                \qquad
                \forall (x, y), (\other{x}, \other{y}) \in \gph \partial (-f)^* \cap (Y \times Y).\numberthis\label{eq:cor:strcvx:1}
            \end{align*}
            Moreover, since $-f$ is continuous and convex, we have by 
            \cite[Prop. 11.3]{rockafellar2009Variational} that 
            \(
                \partial (-f)^* = (\partial (-f))^{-1}
            \),
            so that \eqref{eq:cor:strcvx:1} is equivalent to
            \begin{align*}
                \inner{y - \other{y}, x - \other{x}} \leq -\tfrac{1}{\ell} \nrm{y - \other{y}}^2, \quad \forall (x, y), (\other{x}, \other{y}) \in \graph \partial (-f) \cap (Y \times Y).\numberthis\label{eq:cor:strcvx:2}
            \end{align*}
            Finally, since $-f$ is finite and convex, it follows from \cite[Cor. 9.21]{rockafellar2009Variational} that \(\partial f(\bar{x}) \subseteq - \partial (-f)(\bar{x})\), \(\forall \bar{x} \in \R^n\), so that
            \begin{align*}
                \inner{y - \other{y}, x - \other{x}} \geq \tfrac{1}{\ell} \nrm{y - \other{y}}^2, \quad \forall (x, y), (\other{x}, \other{y}) \in \graph \partial f \cap (Y \times Y).
            \end{align*}
        \end{proofitemize}
    \end{proof}
\end{proposition}

% \begin{proposition}[functions with upper and lower curvature]\label{prop:curvature}
%     Let \(\sigma, \ell \in \R\) and let $Y \subseteq \R^n$ be a closed, linear subspace. Consider a proper lsc function \(f:\R^n \to \Rinf\). 
%     % Consider a proper lsc function \(f:\R^n \to \Rinf\). 
%     % If \(f\in \mathcal F_{\sigma, X}^{\ell, Y}(\R^n)\), then, ...
%     Then, the following hold.
%     \begin{enumerate}
%         \item \label{prop:hypo:cvx} If \(f\) has lower curvature \(\sigma\) on $Y$, then
%         \[
%             \inner{x - \other{x}, \proj_Y(y - \other{y})} \geq \sigma \nrm{\proj_Y(x - \other{x})}^2, \qquad \forall (x,y), (\other{x}, \other{y}) \in \gph \partial f.
%         \]

%         \item \label{prop:hypo:ccv} If \(f\) has upper curvature \(\ell < 0\) on $Y$, then
%         \[
%             \inner{x - \other{x}, \proj_Y(y - \other{y})} \geq \tfrac{1}{\ell} \nrm{\proj_Y(y - \other{y})}^2, \qquad \forall (x,y), (\other{x}, \other{y}) \in \gph \partial f.
%         \]
%     \end{enumerate}
%     \begin{proof}
%         \begin{proofitemize}
%             \item \ref{prop:hypo:cvx}: Let $Z$ be an orthogonal basis for $Y$. Then, $f \circ Z$ has has lower curvature \(\sigma\), and thus it follows from \cite[Prop. 4.15(i)]{evens2023convergence} that $\partial (f \circ Z)$ is $(\sigma, 0)$-semimonotone. Since $\partial (f \circ Z) = Z^\top \circ \partial f \circ Z$, this implies that 
%             \[
%                 \inner{u - \other{u}, v - \other{v}} \geq \sigma \nrm{u - \other{u}}^2, \qquad \forall (u,v), (\other{u}, \other{v}) \in \gph Z^\top \circ \partial f \circ Z.
%             \]
%             which is equivalent to
%             \[
%                 \inner{u - \other{u}, Z^\top(y - \other{y})} \geq \sigma \nrm{u - \other{u}}^2, \qquad \forall (u,y), (\other{u}, \other{y}) \in \gph \partial f \circ Z.
%             \]
            
%             % Noting that $Z^\top Z = \I$, this is equivalent to
%             % \[
%             %     \inner{Z(u - \other{u}), Z(v - \other{v})} \geq \sigma \nrm{Z(u - \other{u})}^2, \qquad \forall (u,v), (\other{u}, \other{v}) \in \gph Z^\top \circ \partial f \circ Z.
%             % \]
%             % Finally, defining $x \coloneqq Zu$, $\other{x} \coloneqq Z\other{u}$, $Zv = Z Z^\top y$, $Z\other{v} = Z Z^\top \other{y}$ and observing that $Z Z^\top = \proj_Y$, the claim is established.
%             \item \ref{prop:hypo:ccv}: 
            
%             By \cite[Prop. 12.60]{rockafellar2009Variational} and strong convexity of $-f$, the conjugate $(-f)^*$ is $-\tfrac{1}{\ell}$\hyp{}smooth, i.e.
%             \begin{align*}
%                 \inner{\nabla (-f)^*(x) - \nabla (-f)^*(\other{x}), x - \other{x}} \leq -\tfrac{1}{\ell} \nrm{x - \other{x}}^2, \quad \forall x, \other{x} \in \R^n.\numberthis\label{eq:cor:strcvx:1}
%             \end{align*}
%             Moreover, since $-f$ is continuous and convex, we have by 
%             \cite[Prop. 11.3]{rockafellar2009Variational} that 
%             \(
%                 \nabla (-f)^* = (\partial (-f))^{-1}
%             \),
%             so that \eqref{eq:cor:strcvx:1} is equivalent to
%             \begin{align*}
%                 \inner{y - \other{y}, x - \other{x}} \leq -\tfrac{1}{\ell} \nrm{y - \other{y}}^2, \quad \forall (x, y), (\other{x}, \other{y}) \in \graph \partial (-f).\numberthis\label{eq:cor:strcvx:2}
%             \end{align*}
%             Finally, since $-f$ is finite and convex, it follows from \cite[Cor. 9.21]{rockafellar2009Variational} that \(\partial f(\bar{x}) \subseteq - \partial (-f)(\bar{x})\), \(\forall \bar{x} \in \R^n\), so that
%             \begin{align*}
%                 \inner{y - \other{y}, x - \other{x}} \geq \tfrac{1}{\ell} \nrm{y - \other{y}}^2, \quad \forall (x, y), (\other{x}, \other{y}) \in \graph \partial f \subseteq - \graph \partial (-f).
%             \end{align*}

%             \item \ref{prop:ccv}: Consider the function 
%             \(\varphi = f - \tfrac{\alpha}2\|\cdot\|^2\). Then, by definition \(\varphi\in\mathcal F^{\ell - \alpha}(\R^n)\), implying that \(\partial \varphi\) is \((0, \tfrac{1}{\ell - \alpha})\)-semimonotone owing to \Cref{prop:hypo:ccv} since \(\alpha>\ell\). Since \(\partial f= \partial \varphi + \alpha \id\), \cite[Ex. 8.8(c)]{Rockafellar1970Convex},  it follows from \Cref{cor:sum:identity} that for \(c > \tfrac{1}{\alpha - \ell}\)  the claimed semimonotonicity holds. 
    
%             \item \ref{prop:hypo:dif+}, \ref{prop:hypo:dif-}:
%             Suppose that \(\ell>\sigma\), since if \(\ell = \sigma\), then, \(\nabla f = \ell \id\) and the claims follow trivially.
%             Consider the function \(\varphi = f - \tfrac{\sigma}2\|\cdot\|^2 \in \mathcal F^{\ell - \sigma}_0(\R^n)\).
%             % for which by definition it holds that $\varphi \in \mathcal F^{\ell - \sigma}_0(\R^n)$.
%             % \subseteq \mathcal F^{\ell - \sigma}_{-(\ell - \sigma)}(\R^n)$.
%             Since $\varphi$ is finite and convex its subdifferential 
%             $\partial \varphi(x)$ is nonempty for all $x \in \R^n$ \cite[Thm. 23.4]{Rockafellar1970Convex}. Consequently, $\varphi$ is continuously differentiable due to \cite[Lem. 2.1]{themelis2020DouglasRachford} and $\nabla \varphi$ is \((0, \tfrac{1}{\ell-\sigma})\)\hyp{}semimonotone due to \cite[Thm. 2.1.10]{nesterov2004introductory}.
%             Therefore, by \cref{prop:calculus:inverse}, there exists a monotone mapping \(\tilde A\) for which
%             \(
%             (\nabla \varphi)^{-1} = \tilde A + \tfrac{1}{\ell-\sigma}
%             \) and thus, owing to $\nabla f = \nabla \varphi + \sigma \id$ \cite[Ex. 8.8(c)]{rockafellar2009Variational} it holds that 
%             \ifspringer
%                 \(
%                     \nabla f 
%                     {}={}
%                     \nabla \varphi + \sigma \id 
%                     {}={}
%                     \big(\tilde A + \tfrac{1}{\ell-\sigma}\id \big)^{-1} + \sigma \id.
%                 \)
%             \else
%                 \[
%                     \nabla f 
%                     {}={}
%                     \nabla \varphi + \sigma \id 
%                     {}={}
%                     \big(\tilde A + \tfrac{1}{\ell-\sigma}\id \big)^{-1} + \sigma \id.
%                 \]
%             \fi
%             The claimed results from \Cref{prop:hypo:dif+,prop:hypo:dif-} then follow from \cref{cor:sem2mon}, where we let $\xi = \tfrac{1}{\ell - \sigma}$ and $\nu = \sigma$. This is because \(\ell - \sigma > 0\) and therefore $1 + 2\xi\nu > 0$ (resp. $\leq 0$) if and only if $\sigma + \ell > 0$ (resp. $\leq 0$).
%             \qedhere
%         \end{proofitemize}
%     \end{proof}
% \end{proposition}

==> TeX/Text/deprecated/deprecated.tex <==

\begin{example}
 In \Cref{lem:partialinverse:comon}, let \(S=A\in\R^{n\times n}\) be a symmetric and invertible linear mapping. Suppose, first that \(\nuP=0\). Due to linearity, condition \eqref{eq:PIlem:cond} can be equivalently represented by
  \(
    A + (\theta-\nuD) P_{X^\bot} \succeq 0.
  \) 
  Therefore, \(A\) may have negative eigenvalues inasmuch as the corresponding eigenvectors lie in \(X^\bot\). 

  Next, suppose that \(\nuD=0\). Let \(\lambda_i\) and \(q_i\), \(i\in\mathcal I\subseteqq [N]\), denote negative eigenvalues of \(A\) and the corresponding eigenvectors. Then, condition \eqref{eq:PIlem:cond} is equivalent to 
  \(
    W \coloneqq A  -\nuD A P_{X} A \succeq 0.
  \)
  Transforming \(W\) using similarity transformation with \(A\) yields the similar matrix
  \(
    A^{-1}  -\nuD P_{X}
  \)
  that shares the same eigenvalues of \(W\). Therefore, \(W\) is positive definite provided that \(q_i\in X\) and \(\nuD \leq \nicefrac{1}{\lambda_i}\). 

  \hl{The second case would not make sense in the context of minimization since the problem would be unbounded below along such eigenvectors...We should probably consider minimax here....Can we have an example in the minimax setup?}
  
\end{example}

\begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin}
    Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\sigma_{A,X}, \rho_{A,X}\in\R\), \ie, 
    \begin{equation}\label{eq:PIlemlin:X}
      \langle x, Ax \rangle 
        {}\geq{}
      \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
    \end{equation}  
    Let \(\bar{A} \dfn A^\top \proj_X A\) and define
    \[
      \alpha
        \dfn
      \lambda_{\rm min}(\proj_{X}(\rho_{A,X} A^\top A -\nuP \bar{A}) \proj_{X})
      ,
      \quad
      \beta
        \dfn
      \nrm{\proj_{X}(A_S - \nuP \bar{A})\proj_{X^\bot}}
      ,
      \quad
      \gamma
        \dfn
      \lambda_{\rm min}(\proj_{X^\bot}(A_S - \nuP \bar{A})\proj_{X^\bot}).
    \]
    Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). 
    Suppose that \(\sigma_{A,X} + \alpha > 0\).
    Then, \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
    \begin{align}
      \theta
        {}\geq{}
      \tfrac{\beta^2}{\sigma_{A,X} + \alpha} + \nuD - \gamma.
      \label{eq:PIlemlin:theta}
    \end{align}
    \begin{proof}
      Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
      \begin{align*}
        V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\|\proj_{X^{\bot}}(w)\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}
          {}\geq{}&
        0.
      \end{align*}
      The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = u + v\) where \(u = \proj_X(w)\) and \(v= \proj_{X^\bot}(w)\). This implies that 
      \(
        \|w\|^2 
          {}={}
        \|u\|^2 + \|v\|^2
      \),
      \begin{align*}
        \langle w,Aw\rangle
          % {}={}&
        % \langle u+v,A(u+v)\rangle 
        % \\
          {}={}&
        \langle u,A u\rangle + 2\langle u,A_S v\rangle + \langle v,Av\rangle
      \end{align*}
      and
      \[
        \|\proj_{X}(Aw)\|^{2} = \inner{w, \bar{A} w} = \inner{u, \bar{A} u} + 2\inner{u, \bar{A} v} + \inner{v, \bar{A} v}
      \]
      Therefore,
      \begin{align*}
        V(w)
          {}={}&
        (\theta-\nuD)\|v\|^2 + \langle u,Au\rangle - \nuP\inner{u, \bar{A} u} + \langle v,(A - \nuP \bar{A})v\rangle + 2\langle u,(A_S - \nuP \bar{A}) v\rangle\\
        \dueto{\eqref{eq:elicit:lin:X}}
          {}\geq{}&
        (\theta-\nuD)\|v\|^2 + \sigma_{A,X} \|u\|^2 + \rho_{A,X}\|Au\|^2 - \nuP \inner{u,\bar{A} u} + 2\langle u,(A_S - \nuP \bar{A}) v\rangle + \langle v,(A - \nuP \bar{A})v\rangle \\
            {}={}&
        (\theta-\nuD)\|v\|^2 + \sigma_{A,X} \|u\|^2 + \inner{u,(\rho_{A,X} A^\top A - \nuP \bar{A}) u} + 2\langle u,(A_S- \nuP \bar{A}) v\rangle + \langle v,(A - \nuP \bar{A})v\rangle
          \numberthis\label{eq:PIlemlin:ineq}
      \end{align*}
      % where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle u, Av \rangle\). Setting $\varepsilon = 2\rho_{A,X} > 0$ yields
      % \begin{align*}
      %   V(w)
      %     {}\geq{}&
      %   \sigma_{A,X} \|v\|^2 + \langle u,(A - \nuP \bar{A})u\rangle + \langle v,(A - 2\nuP \bar{A}) u\rangle + (\theta-\nuD - \tfrac{1}{4\rho_{A,X}})\|u\|^2 - \nuP \inner{v,\bar{A} v}
      %     \numberthis \label{eq:PIlemlin:ineq}
      % \end{align*}
      We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality, i.e.,
      \begin{align*}
        \inner{u,(\rho_{A,X} A^\top A - \nuP \bar{A}) u}
          {}={}
        \inner{u,\proj_{X}(\rho_{A,X} A^\top A -\nuP \bar{A}) \proj_{X} u}
          {}\geq{}
        \alpha\|u\|^2,
        \numberthis\label{eq:PIlemlin:b1}
      \end{align*} 
      where the equality follows by orthogonality between \(X\) and \(X^\bot\). Similarly,
      \begin{align*}
        \langle u,(A_S - \nuP \bar{A}) v\rangle
          {}={}
        \langle u,\proj_{X}(A_S - \nuP \bar{A})\proj_{X^\bot} v\rangle
          {}\geq{}
        -\beta\|u\|\|v\|
        \numberthis\label{eq:PIlemlin:b2}
      \end{align*} 
      and
      \begin{align*}
        \langle v,(A - \nuP \bar{A})v\rangle
          {}={}
        \langle v,\proj_{X^\bot}(A - \nuP \bar{A})\proj_{X^\bot}v\rangle
          {}\geq{}
        \gamma\|v\|^2.
        \numberthis\label{eq:PIlemlin:b3}
      \end{align*} 
      Using ~\eqref{eq:PIlemlin:b1},~\eqref{eq:PIlemlin:b2} and ~\eqref{eq:PIlemlin:b3} to lower bound~\eqref{eq:PIlemlin:ineq} yields
      \begin{align*}
        V(w)
          {}\geq{}&
          (\sigma_{A,X} + \alpha) \|u\|^2 - 2 \beta\|u\|\|v\| + (\theta-\nuD+\gamma)\|v\|^2.
      \end{align*}
      Assuming $\theta-\nuD+\gamma \geq 0$ as in~\eqref{eq:PIlemlin:theta} and using the Fenchel-Young inequality, we obtain
      \(
        V(w) 
          {}\geq{}
        (\sigma_{A,X} + \alpha - \tfrac{\beta^2}{\theta-\nuD+\gamma})\|u\|^2, 
      \)
      which is positive owing to~\eqref{eq:PIlemlin:theta}. 
    \end{proof}
  \end{lemma}
  
  \begin{example}
    In \Cref{lem:partialinverse:comon:lin}, let \(A\in\R^{n\times n}\) be a symmetric and invertible linear mapping and let \(\rho_{A,X} = \nuP= \nuD = 0\). Then,
    \[
      \alpha
        =
      0
      ,
      \quad
      \beta
        \dfn
      \nrm{\proj_{X}A_S\proj_{X^\bot}}
      ,
      \quad
      \gamma
        \dfn
      \lambda_{\rm min}(\proj_{X^\bot}A_S\proj_{X^\bot}).
    \]  
    Therefore, \cite[Thm. 5]{rockafellar2019Progressive} is recovered, since
    \(\lambda_{\rm min}(\proj_{X^\bot}A_S\proj_{X^\bot}) \geq -\nrm{\proj_{X^\bot}A_S\proj_{X^\bot}} \geq -\nrm{\proj_{X^\bot}A\proj_{X^\bot}}\)
  \end{example}
  
  % \begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin:2}
  %   Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
  %   \begin{equation}\label{eq:PIlemlin:X:2}
  %     \langle x, Ax \rangle 
  %       {}\geq{}
  %     \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
  %   \end{equation}  
  %   Let \(b_i= \|B_i\|\), \(i=1,2,3\), where the matrices \(\alpha,B_2,B_3\in\R^{n\times n}\) are defined by 
  %   \begin{align*}
  %     \alphaw
  %       {}\coloneqq{}&
  %     \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
  %     \quad
  %     B_2w
  %       {}\coloneqq{}
  %     \proj_{X}\big(A\proj_{X^\bot}(w)\big),
  %     \quad
  %     B_3w
  %       {}\coloneqq{}
  %     \proj_{X}\big(Aw\big),  \quad w \in \R^n.
  %     % \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
  %   \end{align*}
  %   Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). Suppose that $\nuP \leq 0$ Then, 
  %   % \(T^X\) is \(V\)-oblique comonotone if
  %   \begin{enumerate}
  %     \item If \(\rho_{A,X}>0\), then \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
  %     \begin{align}
  %       c
  %         {}\geq{}
  %        0, \quad  
  %       % \label{eq:elicit:lin:rho}
  %       % \\
  %       0
  %         {}\leq{}
  %         \sigma_{A,X}-\nuPb_3^2 - \tfrac{b^2_2}{4c}
  %       \label{eq:PIlemlin:theta:2}
  %     \end{align}
  %     where $c \dfn \theta-\nuD-\nuPb_3^2-\tfrac{1}{4\rho_{A,X}}-\alpha$.
  %     \item If \(\rho_{A,X}=0\), \bhl{TODO}
  %   \end{enumerate}
  %   \bhl{Note: Here, we dealt with the final term through the introduction of $b_3$, allowing for potentially negative $\sigma_{A,X}$. However, it still isn't nice...}
  %   \begin{proof}
  %     Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
  %   \begin{align*}
  %     V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\langle w,\proj_{X^{\bot}}(w)\rangle - \nuP\|\proj_{X}(Aw)\|^{2}
  %        {}\geq{}&
  %      0.
  %   \end{align*}
  %   The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This implies that 
  %   \(
  %     \|w\|^2 
  %       {}={}
  %     \|v\|^2 + \|u\|^2,
  %   \)
  %   and
  %   \begin{align*}
  %     \langle w,Aw\rangle
  %       {}={}&
  %     \langle u+v,A(u+v)\rangle 
  %     \\
  %       {}={}&
  %     % \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
  %     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle
  %   \end{align*}
  %   First, consider the case when \(\rho_{A,X} > 0\). Then, it follows that
  %   \begin{align*}
  %     V(w)
  %       {}={}&
  %     % \langle v,Av\rangle + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
  %     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
  %     % \dueto{$(\nuP \leq 0)$}
  %       {}\geq{}&
  %       % \langle v,Av\rangle + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2\\
  %       \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 \textcolor{red}{- \nuPb_3^2\|w\|^{2}}\\
  %     \dueto{\eqref{eq:elicit:lin:X}}
  %       {}\geq{}&
  %       % \sigma_{A,X} \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2
  %       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD-\nuPb_3^2)\|u\|^2\\
  %       {}\geq{}&
  %       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,Au\rangle - \tfrac{\varepsilon}{2}\|Av\|^2 - \tfrac{1}{2\varepsilon}\|u\|^2+ (\theta-\nuD-\nuPb_3^2)\|u\|^2
  %   \end{align*}
  %   where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle u, Av \rangle\). Setting $\varepsilon = 2\rho_{A,X} > 0$ yields
  %   \begin{align*}
  %     V(w)
  %       {}\geq{}&
  %       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 + \langle u,Au\rangle + \langle v,Au\rangle + (\theta-\nuD-\nuPb_3^2 - \tfrac{1}{4\rho_{A,X}})\|u\|^2
  %       \numberthis \label{eq:PIlemlin:ineq:2}
  %   \end{align*}
  
  %   We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality.
  %   \begin{align*}
  %     \langle u, Au \rangle 
  %       {}={}
  %     \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     - \alpha\|u\|^2   
  %     \numberthis \label{eq:PIlemlin:b1:2}
  %    \end{align*} 
  %    where the equality follows by orthogonality between \(X\) and \(X^\bot\). Similarly,
  %   %  \begin{align*}
  %   %   \langle v, (A+A^\top)u \rangle 
  %   %    {}={}
  %   %  \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
  %   %    {}\geq{}
  %   %  -b_2\|u\|\|v\|,    
  %   % %  \numberthis \label{eq:elicit:lin:b2}
  %   % \end{align*}
  %   \begin{align*}
  %     \langle v, Au \rangle 
  %       {}={}
  %     \langle v, \proj_{X}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %       -b_2\|u\|\|v\|. 
  %     \numberthis \label{eq:PIlemlin:b2:2}
  %    \end{align*} 
  %    Using ~\eqref{eq:PIlemlin:b1:2} and~\eqref{eq:PIlemlin:b2:2} to lower bound~\eqref{eq:PIlemlin:ineq:2} yields
  %    \begin{align*}
  %     V(w)
  %       {}\geq{}&
  %       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 - b_2\|u\|\|v\| + c\|u\|^2
  %   \end{align*}
  %   where
  %    \(
  %       c 
  %         {}\coloneqq{}
  %       \theta-\nuD-\nuPb_3^2-\tfrac{1}{4\rho_{A,X}}-\alpha
  %    \). 
  %    Assuming $c \geq 0$ as in~\eqref{eq:PIlemlin:theta:2}, and using the Fenchel-Young inequality we obtain
  %    \(
  %     V(w) \geq (\sigma_{A,X}-\nuPb_3^2 - \tfrac{b^2_2}{4c})\|v\|^2, 
  %    \)
  %    which is positive owing to~\eqref{eq:PIlemlin:theta:2}. 
  %   \end{proof}
  % \end{lemma}
  
  % \begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin:3}
  %   Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
  %   \begin{equation}\label{eq:PIlemlin:X:3}
  %     \langle x, Ax \rangle 
  %       {}\geq{}
  %     \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
  %   \end{equation}  
  %   Let \(b_i= \|B_i\|\), \(i=1,2\), where the matrices \(\alpha,B_2\in\R^{n\times n}\) are defined by 
  %   \begin{align*}
  %     \alphaw
  %       {}\coloneqq{}&
  %     \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
  %     \qquad
  %     B_2w
  %       {}\coloneqq{}
  %     \proj_{X}\big(A\proj_{X^\bot}(w)\big),  \qquad w \in \R^n.
  %     % \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
  %   \end{align*}
  %   Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). Suppose that $\nuP \leq 0$ Then, 
  %   % \(T^X\) is \(V\)-oblique comonotone if
  %   \begin{enumerate}
  %     \item If \(\rho_{A,X}>0\), then \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
  %     \begin{align}
  %       c
  %         {}\geq{}
  %        0, \quad  
  %       % \label{eq:elicit:lin:rho}
  %       % \\
  %       0
  %         {}\leq{}
  %      \sigma_{A,X} - \tfrac{b^2_2}{4c}
  %       \label{eq:PIlemlin:theta:3}
  %     \end{align}
  %     where $c \dfn \theta-\nuD-\tfrac{1}{4\rho_{A,X}}-\alpha$.
  %     \item If \(\rho_{A,X}=0\), \bhl{TODO}
  %   \end{enumerate}
  %   \begin{proof}
  %     Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
  %   \begin{align*}
  %     V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\langle w,\proj_{X^{\bot}}(w)\rangle - \nuP\|\proj_{X}(Aw)\|^{2}
  %        {}\geq{}&
  %      0.
  %   \end{align*}
  %   The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This implies that 
  %   \(
  %     \|w\|^2 
  %       {}={}
  %     \|v\|^2 + \|u\|^2,
  %   \)
  %   and
  %   \begin{align*}
  %     \langle w,Aw\rangle
  %       {}={}&
  %     \langle u+v,Aw\rangle 
  %     \\
  %       {}={}&
  %     % \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
  %     \langle v,Aw\rangle+\langle u,A u\rangle+\langle u,Av\rangle
  %   \end{align*}
  %   First, consider the case when \(\rho_{A,X} > 0\). Then, it follows that
  %   \begin{align*}
  %     V(w)
  %       {}={}&
  %     \langle v,Aw\rangle+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
  %       {}={}&
  %       \langle v,\proj_X(Aw)\rangle+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
  %       {}\geq{}&
  %       - \tfrac{1}{2\varepsilon}\|v\|^2 - \tfrac{\varepsilon}{2}\|\proj_X(Aw)\|^2+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}
  %   \end{align*}
  %   where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle v,\proj_X(Aw)\rangle\). Setting $\varepsilon = -2\nuP > 0$ yields
  %   \begin{align*}
  %     V(w)
  %       {}\geq{}&
  %       \tfrac{1}{4\nuP}\|v\|^2+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2
  %   \end{align*}
  %   ???
  %   \end{proof}
  % \end{lemma}
  
  % \begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin:3}
  %   Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
  %   \begin{equation}\label{eq:PIlemlin:X:3}
  %     \langle x, Ax \rangle 
  %       {}\geq{}
  %     \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
  %   \end{equation}  
  %   Let \(b_i= \|B_i\|\), \(i=1,2\), where the matrices \(\alpha,B_2\in\R^{n\times n}\) are defined by 
  %   \begin{align*}
  %     \alphaw
  %       {}\coloneqq{}&
  %     \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
  %     \qquad
  %     B_2w
  %       {}\coloneqq{}
  %     \proj_{X}\big(A\proj_{X^\bot}(w)\big),  \qquad w \in \R^n.
  %     % \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
  %   \end{align*}
  %   Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). Suppose that $\nuP \leq 0$ Then, 
  %   % \(T^X\) is \(V\)-oblique comonotone if
  %   \begin{enumerate}
  %     \item If \(\rho_{A,X}>0\), then \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
  %     \begin{align}
  %       c \dfn \theta-\nuD - \tfrac{1}{8\rho_{A,X}} - \alpha
  %         {}\geq{}
  %        0, \quad  
  %       % \label{eq:elicit:lin:rho}
  %       % \\
  %       0
  %         {}\leq{}
  %       2\sigma_{A,X}+ \tfrac{1}{4\nuP} - \tfrac{b^2_2}{4c}
  %       \label{eq:PIlemlin:theta:3}
  %     \end{align}
  %     where $c \dfn \theta-\nuD-\tfrac{1}{4\rho_{A,X}}-\alpha$.
  %     \item If \(\rho_{A,X}=0\), \bhl{TODO}
  %   \end{enumerate}
  %   \begin{proof}
  %     Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
  %   \begin{align*}
  %     V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\langle w,\proj_{X^{\bot}}(w)\rangle - \nuP\|\proj_{X}(Aw)\|^{2}
  %        {}\geq{}&
  %      0.
  %   \end{align*}
  %   The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This implies that 
  %   \(
  %     \|w\|^2 
  %       {}={}
  %     \|v\|^2 + \|u\|^2,
  %   \)
  %   and
  %   \begin{align*}
  %     \langle w,Aw\rangle
  %       {}={}&
  %     \langle u+v,A(u+v)\rangle 
  %     \\
  %       {}={}&
  %     % \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
  %     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle
  %   \end{align*}
  %   First, consider the case when \(\rho_{A,X} > 0\). Then, it follows that
  %   \begin{align*}
  %     V(w)
  %       {}={}&
  %       \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
  %       {}\geq{}&
  %       \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 + \langle v,\proj_{X}(Aw)\rangle + \tfrac{1}{4\nuP}\|v\|^{2}
  %   \end{align*}
  %   where the Fenchel-Young inequality was used to control the inner product \(\langle v,\proj_X(Aw)\rangle\). Since $\langle v,\proj_{X}(Aw)\rangle = \langle v,Aw\rangle$, it follows that
  %   \begin{align*}
  %     V(w)
  %       {}\geq{}&
  %       2\langle v,Av\rangle+\langle u,A u\rangle+2\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 + \tfrac{1}{4\nuP}\|v\|^{2}\\
  %     \dueto{\eqref{eq:elicit:lin:X}}
  %       {}\geq{}&
  %       % \sigma_{A,X} \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2
  %       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 + 2\rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + 2\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2\\
  %       {}\geq{}&
  %       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 + 2\rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + 2\langle v,Au\rangle - \tfrac{\varepsilon}{2}\|Av\|^2 - \tfrac{1}{2\varepsilon}\|u\|^2+ (\theta-\nuD)\|u\|^2
  %   \end{align*}
  %   where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle u, Av \rangle\). Setting $\varepsilon = 4\rho_{A,X} > 0$ yields
  %   \begin{align*}
  %     V(w)
  %       {}\geq{}&
  %       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 + \langle u,Au\rangle + 2\langle v,Au\rangle + (\theta-\nuD - \tfrac{1}{8\rho_{A,X}})\|u\|^2
  %       \numberthis \label{eq:PIlemlin:ineq:3}
  %   \end{align*}
  
  %   We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality.
  %   \begin{align*}
  %     \langle u, Au \rangle 
  %       {}={}
  %     \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     - \alpha\|u\|^2   
  %     \numberthis \label{eq:PIlemlin:b1:3}
  %    \end{align*} 
  %    where the equality follows by orthogonality between \(X\) and \(X^\bot\). Similarly,
  %   %  \begin{align*}
  %   %   \langle v, (A+A^\top)u \rangle 
  %   %    {}={}
  %   %  \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
  %   %    {}\geq{}
  %   %  -b_2\|u\|\|v\|,    
  %   % %  \numberthis \label{eq:elicit:lin:b2}
  %   % \end{align*}
  %   \begin{align*}
  %     \langle v, Au \rangle 
  %       {}={}
  %     \langle v, \proj_{X}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %       -b_2\|u\|\|v\|. 
  %     \numberthis \label{eq:PIlemlin:b2:3}
  %    \end{align*} 
  %    Using ~\eqref{eq:PIlemlin:b1:3} and~\eqref{eq:PIlemlin:b2:3} to lower bound~\eqref{eq:PIlemlin:ineq:3} yields
  %    \begin{align*}
  %     V(w)
  %       {}\geq{}&
  %       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 - b_2\|u\|\|v\| + c\|u\|^2
  %   \end{align*}
  %   where
  %    \(
  %       c 
  %         {}\coloneqq{}
  %       \theta-\nuD - \tfrac{1}{8\rho_{A,X}} - \alpha
  %    \). 
  %    Assuming $c \geq 0$ as in~\eqref{eq:PIlemlin:theta:3}, and using the Fenchel-Young inequality we obtain
  %    \(
  %     V(w) \geq (2\sigma_{A,X}+ \tfrac{1}{4\nuP} - \tfrac{b^2_2}{4c})\|v\|^2, 
  %    \)
  %    which is positive owing to~\eqref{eq:PIlemlin:theta:3}. 
  %   \end{proof}
  % \end{lemma}
  
  \bhl{TODO: the remainder of this note contains old results which might be relevant, need to fix refs}
  The general inclusion problem \eqref{eq:DRS problem} may be equivalently cast as a linkage problem by introducing auxiliary variables as follows. 
  \begin{align*}
    0 
      {}\in{}
    Ax_1 + B x_1
      {}\iff{}&
    0 
      {}\in{}
    Ax_1 + y_2,
    \quad
    0
      {}\in{}
    Bx_1 - y_2
    \\
    {}\iff{}&
    x= (x_1,x_2)
      {}\in{}
    X,
    \quad
    y=(y_1,y_2) 
      {}\in{}
    X^\bot
    ,\quad 
    y
      {}\in{}
    {\hat T}x,
  \end{align*}
  where 
  \[
    \hat T x
      {}={}
    (Ax_1, Bx_2),
    \quad 
    X= \set{x=(x_1,x_2)\in \R^{2n}}[x_1 = x_2]. 
  \]
  Leveraging the idea of elicitation, operator \(\hat T\) in the above inclusion above may be replaced by \({\hat T}x + \theta \proj_{X^\bot}(x)\) for any \(\theta \in[0,\infty)\) without affecting the solutions of the inclusion. 
   Further noting that 
  \(
    \proj_X(x) = \big(\tfrac12 (x_1 + x_2), \tfrac12 (x_1 + x_2) \big),
  \)
  leads to the following equivalent problem 
  \[
    x= (x_1,x_2)
      {}\in{}
    X,
    \quad
    y=(y_1,y_2) 
      {}\in{}
    X^\bot
    ,\quad 
    y
      {}\in{}
    \left(%
      Ax_{1} + \tfrac{\theta}{2}(x_{1}+x_{2}), 
      Bx_{2}  + \tfrac{\theta}{2}(x_{1}+x_{2})
    \right).
  \]
  
  
  \hl{TODO: Elicitation preliminaries}
  
    \begin{lemma}\label{lem:elicit:linear}
        Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
        \begin{equation}\label{eq:elicit:lin:X}
            \langle Ax, x \rangle 
              {}\geq{}
            \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
          \end{equation}  
        Let \(b_i= \|B_i\|\), \(i=1,2\), where the matrices \(B_1,B_2\in\R^{n\times n}\) are defined by 
    \begin{align*}
      B_1w
        {}\coloneqq{}&
      \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
      \qquad
      B_2w
        {}\coloneqq{}
      \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
    \end{align*}
    Suppose that \(\sigma_A < \sigma_{A,X}\). Then,
    \begin{enumerate}
      \item If \(\rho_{A,X}>0\), then \(A\) has elicitable \((\sigma_A,\rho_A)\)-semimonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
    \begin{align}
      \rho_A 
        {}\leq{}
      0, \quad  
      % \label{eq:elicit:lin:rho}
      % \\
      0
        {}\leq{}
    -\rho_{A}\left(1+\tfrac{\rho_{A}}{\rho_{A,X}}\right)\theta^{2}
        {}+{}
      (1+2\rho_{A}b_{1})\theta
        {}+{}
      \tfrac{b_{2}^{2}}{4\sigma_{A}^{\prime}}-\sigma_{A}-b_{1}
      \label{eq:elicit:lin:theta}
    \end{align}
    \item If \(\rho_{A,X}=0\) then \(A\) has elicitable \((\sigma_A,0)\)-semimonotonicity (everywhere) at level \(\theta \geq \sigma_A + b_1 + \tfrac{b_2^2}{4(\sigma_{A,X}-\sigma_A)}\). 
    \end{enumerate}
    \begin{proof}
      A given vector \(w\in\R^n\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This would imply that 
      \(
        \|w\|^2 
          {}={}
        \|v\|^2 + \|u\|^2,
      \)
      and 
      \begin{align*}
        \|Aw+\theta\proj_{X^{\top}}(w)\|^{2}
          {}={}&
        \|Aw\|^{2}+\theta^{2}\|\proj_{X^{\top}}(w)\|^{2}+2\langle Aw,\theta\proj_{X^{\top}}(w)\rangle
        \\
          {}={}&
        \|Aw\|^{2}+\theta^{2}\|u\|^{2}+2\theta\langle Av+Au,u\rangle.
        \numberthis \label{eq:elicit:1}
      \end{align*}
      The mapping \(A+ \theta \proj_{X^\bot}\) is linear. Therefore, to establish the claim it suffices to show that for all \(w\in\R^n\) the following holds for some \(\rho_A, \sigma_A\leq0\):
      \begin{align*}
        V(w) \coloneqq \langle w,Aw+\theta\proj_{X^{\top}}(w)\rangle-\sigma_{A}\|w\|^{2} - \rho_{A}\|Aw+\theta\proj_{X^{\top}}(w)\|^{2} \geq 0. 
      \end{align*}
      Note that 
      \begin{align*}
        \langle w,Aw+\theta \proj_{X^\bot}(w)\rangle
          {}={}&
        \langle u+v,A(u+v)+\theta u\rangle 
        \\
          {}={}&
        \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
          {}+{}
        \theta \|u\|^2
      \end{align*}
      First, consider the case when \(\rho_{A,X} > 0\). Combine this with \eqref{eq:elicit:1} to obtain
      \begin{align*}
        V(w) 
          {}={}&
        \langle v,Av\rangle-\sigma_{A}\|v\|^{2}-\rho_{A}\|Aw\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
        \\%
          &{}+{}
        \langle v,(A+A^{\top})u\rangle 
          {}+{}
        (1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle
        \numberthis\label{eq:elicit:lin:Aw}
        \\%
        \dueto{\eqref{eq:elicit:lin:X}}
          {}\geq{}&
        -\sigma_{A}^\prime\|v\|^{2}+\rho_{A,X}\|Av\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
        \\%
          &{}+{}
        \langle v,(A+A^{\top})u\rangle 
          {}+{}
        (1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle Av,u\rangle  
        \\%
            {}\geq{}&
        -\sigma_{A}^\prime\|v\|^{2}
          {}+{}
        \rho_{A,X}\|Av\|^{2}
          {}+{}
        (\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
        \\%
          &{}+{}
        \langle v,(A+A^{\top})u\rangle
          {}+{}
        (1-2\rho_{A}\theta)\langle Au,u\rangle+ \tfrac{\rho_{A}\theta}{\varepsilon} \|Av\|^2 + \rho_{A}\theta \varepsilon \|u\|^2  
      \end{align*}
      where \(\sigma_{A}^\prime = \sigma_{A} - \sigma_{A,X}\) and the Fenchel-young inequality was used in the last inequality to control the inner product \(-2\rho_A\theta\langle Av,u \rangle\). 
      Setting \(\varepsilon = -\tfrac{\rho_A \theta}{\rho_{A,X}}>0\) yields 
      \begin{align*}
        V(w) 
          {}={}&
        -\sigma_{A}^\prime\|v\|^{2}
            {}+{}
          \big(%
            \theta-\sigma_{A}-\rho_{A}\theta^{2} - \tfrac{\rho_{A}^2\theta^2}{\rho_{A,X}}
          \big)\|u\|^{2}
          \\%
            &{}+{}
          \langle v,(A+A^{\top})u\rangle
            {}+{}
          (1-2\rho_{A}\theta)\langle Au,u\rangle 
        \numberthis\label{eq:elicit:lin:Vw}
      \end{align*}
        We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality. 
        \begin{align*}
          \langle u, Au \rangle 
            {}={}
          \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
            {}\geq{}
          - b_1\|u\|^2   
          \numberthis \label{eq:elicit:lin:b1}
        \end{align*} 
        where the equality follows by orthogonality between \(X\) and \(X^\bot\). 
        Similarly, 
        \begin{align*}
          \langle v, (A+A^\top)u \rangle 
            {}={}
          \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
            {}\geq{}
          -b_2\|u\|\|v\|,    
          \numberthis \label{eq:elicit:lin:b2}
        \end{align*}
        Using \eqref{eq:elicit:lin:b1}, \eqref{eq:elicit:lin:b2} to lower bound \eqref{eq:elicit:lin:Vw} yields
          \begin{align*}
          V(w) 
            {}\geq{}&
          -\sigma_A^\prime\|v\|^{2} - b_2\|u\|\|v\| + c\|u\|^2
        \end{align*}
        where
        \(
          c 
            {}\coloneqq{}
          \theta-\sigma_{A}-\rho_{A}\theta^{2} - \tfrac{\rho_{A}^2\theta^2}{\rho_{A,X}} -(1-2\rho_{A}\theta)b_{1}
        \). 
        Further noting that \(\sigma_{A}^{\prime}<0\), \(\rho_A\leq0\) as ensured in \eqref{eq:elicit:lin:theta}, and using the Fenchel-Young inequality we obtain
        \(
          V(w) \geq (c + \tfrac{b^2_2}{4\sigma_A^\prime})\|u\|^2, 
        \)
        which is positive owing to \eqref{eq:elicit:lin:theta}. 
        
        In the case where \(\rho_{A,X} = 0\), \eqref{eq:elicit:lin:Aw} simplifies to 
        \begin{align*}
          V(w) 
            {}={}&
          \langle v,Av\rangle-\sigma_{A}\|v\|^{2}+(\theta-\sigma_{A})\|u\|^{2}
          % \\%
            {}+{}
          \langle v,(A+A^{\top})u\rangle 
            {}+{}
          \langle Au,u\rangle.
        \end{align*}
        Following the same steps as above yields the claimed range for \(\theta\). 
  
        \bhl{Could we have used the positive terms \(\|Aw\|^2\) in \eqref{eq:elicit:lin:Aw} to obtain a better parameter range?}
      \end{proof}
    \end{lemma}
  
  
  % \begin{lemma}
  %     Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\), \ie, 
  %     \begin{equation}\label{eq:elicit:lin:X}
  %         \langle Ax, x \rangle 
  %           {}\geq{}
  %         \sigma_{A,X} \|w\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
  %       \end{equation}  
  %     Then, \(A\) has elicitable \((\sigma_A,\rho_A)\)-semi-monotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
  % \begin{align}
  %   \rho_A 
  %     {}\leq{}&
  %    0, \quad \rho_{A}\leq \rho_{A,X}, 
  %   % \\
  %   \quad
  %   % \sigma_{A}^\prime
  %     % {}={}
  %   \sigma_{A} 
  %     {}<{}
  %   \sigma_{A,X},  
  %   \label{eq:elicit:lin:rho}
  %   % \label{eq:elicit:lin:sigma}
  %   \\
  %   0
  %     {}\leq{}&
  %  \left(\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}\right)
  %     {}+{}
  %   \tfrac{1}{(\sigma_{A}-\sigma_{A,X})}\left(\rho_{A}\theta b_{4}+\rho_{A}b_{3}-\tfrac{1}{2}b_{2}\right)^{2}
  %   \label{eq:elicit:lin:theta}
  % \end{align}
  % \hl{TODO: a clean range for theta?...}
  
  % where \(b_i= \|B_i\|\), \(i=1,\cdots,4\), and the matrices 
  %  \(B_1,B_2,B_3,B_4\in\R^{n\times n}\) are define by 
  % \begin{align*}
  %   B_1w 
  %     {}\coloneqq{}&
  %   \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
  %   \qquad
  %   B_2w 
  %     {}\coloneqq{}
  %   \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big),
  %     \\
  %   B_3w 
  %     {}\coloneqq{}&
  %   \proj_{X}\big((A^\top A)\proj_{X^\bot}(w)\big),
  %   \quad
  %   B_4w 
  %     {}\coloneqq{}
  %   \proj_{X}\big(A^\top \proj_{X^\bot}(w)\big).
  % \end{align*}
  % In particular, if \(\rho_{A,X}=0\) then \(A\) has elicitable \((\sigma_A,0)\)-semi-monotone at level \(\theta \geq \sigma_A + b_1 + \tfrac{b_2^2}{4(\sigma_{A,X}-\sigma_A)}\). 
  % \begin{proof}
  %   A given vector \(w\in\R^n\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This would imply that 
  %   \(
  %     \|w\|^2 
  %       {}={}
  %     \|v\|^2 + \|u\|^2,
  %   \)
  %   and 
  %   \begin{align*}
  %     \|Aw+\theta\proj_{X^{\top}}(w)\|^{2}
  %       {}={}&
  %     \|Aw\|^{2}+\theta^{2}\|\proj_{X^{\top}}(w)\|^{2}+2\langle Aw,\theta\proj_{X^{\top}}(w)\rangle
  %     \\
  %       {}={}&
  %     \|Av\|^{2}+\|Au\|^{2}+2\langle Av,Au\rangle+\theta^{2}\|u\|^{2}+2\theta\langle Av+Au,u\rangle.
  %     \numberthis \label{eq:elicit:1}
  %   \end{align*}
  %   The mapping \(A+ \theta \proj_{X^\bot}\) is linear. Therefore, to establish the claim it suffices to show that for all \(w\in\R^n\) the following holds for some \(\rho_A, \sigma_A\leq0\). 
  %   \begin{align*}
  %     V(w) \coloneqq \langle w,Aw+\theta\proj_{X^{\top}}(w)\rangle-\sigma_{A}\|w\|^{2} - \rho_{A}\|Aw+\theta\proj_{X^{\top}}(w)\|^{2} \geq 0. 
  %   \end{align*}
  %   Note that 
  %   \begin{align*}
  %     \langle w,Aw+\theta \proj_{X^\bot}(w)\rangle
  %       {}={}&
  %     \langle u+v,A(u+v)+\theta u\rangle 
  %     \\
  %       {}={}&
  %     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
  %       {}+{}
  %     \theta \|u\|^2
  %   \end{align*}
  %   Combine this with \eqref{eq:elicit:1} to obtain
  %   \begin{align*}
  %     V(w) 
  %       {}={}&
  %     \langle v,Av\rangle-\sigma_{A}\|v\|^{2}-\rho_{A}\|Av\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}-\rho_{A}\|Au\|^{2}
  %     \\%
  %       &{}+{}
  %     \langle v,(A+A^{\top})u\rangle-2\rho_{A}\langle v,A^{\top}Au\rangle+(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle
  %     \\%
  %     \dueto{\eqref{eq:elicit:lin:X}}
  %       {}\geq{}&
  %     -\sigma_{A}^\prime\|v\|^{2}-\rho_{A}^\prime\|Av\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}-\rho_{A}\|Au\|^{2}
  %     \\%
  %       &{}+{}
  %     \langle v,(A+A^{\top})u\rangle-2\rho_{A}\langle v,A^{\top}Au\rangle+(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle  
  %     \\%
  %         {}\geq{}&
  %     -\sigma_{A}^\prime\|v\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
  %     \\%
  %       &{}+{}
  %     \langle v,(A+A^{\top})u\rangle-2\rho_{A}\langle v,A^{\top}Au\rangle+(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle  
  %     \numberthis\label{eq:elicit:lin:Vw}
  %   \end{align*}
  %   where \(\sigma_{A}^\prime = \sigma_{A} - \sigma_{A,X}\) and \(\rho_{A}^\prime =\rho_{A} - \rho_{A,X}\), and \eqref{eq:elicit:lin:rho} was used in the last inequality. 
  
  %   We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality. 
  %   \begin{align*}
  %     \langle u, Au \rangle 
  %       {}={}
  %     \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     - b_1\|u\|^2   
  %     \numberthis \label{eq:elicit:lin:b1}
  %    \end{align*} 
  %    where the equality follows by orthogonality between \(X\) and \(X^\bot\). 
  %    Similarly, 
  %    \begin{align*}
  %      \langle v, (A+A^\top)u \rangle 
  %       {}={}
  %     \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     -b_2\|u\|\|v\|,    
  %     \numberthis \label{eq:elicit:lin:b2}
  %    \end{align*}
  %    and 
  %    \begin{align*}
  %      \langle v, A^\top A u \rangle 
  %       % {}={}
  %     % \langle v, \proj_{X}\big(A^\top A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     -b_3\|u\|\|v\|,
  %     \quad 
  %     \langle v, A^\top u \rangle 
  %       % {}={}
  %     % \langle v, \proj_{X}\big(A^\top \proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     -b_4\|u\|\|v\|. 
  %     \numberthis \label{eq:elicit:lin:b34}
  %    \end{align*}
  %    Using \eqref{eq:elicit:lin:b1}, \eqref{eq:elicit:lin:b2}, \eqref{eq:elicit:lin:b34} to lower bound \eqref{eq:elicit:lin:Vw} yields
  %    % \begin{align*}
  %    %  V(w) 
  %    %    {}\geq{}&
  %    %  -\sigma_{A}^{\prime}\|v\|^{2}+\left(2\rho_{A}\theta b_{4}+2\rho_{A}b_{3}-b_{2}\right)\|u\|\|v\|
  %    %  \\
  %    %    &{}+{}
  %    %  (\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1})\|u\|^{2} 
  %    %  \\
  %    %    {}\geq{}&
  %    %  \big(\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}\big)\|u\|^{2}
  %    % \end{align*}
  %    % 
  %     \begin{align*}
  %     V(w) 
  %       {}\geq{}&
  %     a\|v\|^{2} - 2b\|u\|\|v\| + c\|u\|^2
  %     \\
  %     %   {}\geq{}&
  %     % \big(\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}\big)\|u\|^{2}
  %    \end{align*}
  %    where
  %    \[
  %     a \coloneqq -\sigma_A^\prime,
  %     \quad
  %     b \coloneqq -\rho_{A}\theta b_{4}-\rho_{A}b_{3} + \tfrac12b_{2}, 
  %     \quad
  %     c \coloneqq \theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}.
  %    \]
  %    Further noting that \(\sigma_{A}^{\prime}<0\), \(\rho_A\leq0\) as ensured in \eqref{eq:elicit:lin:rho}, and using the Fenchel-Young inequality we obtain
  %    \(
  %     V(w) \geq (c - \tfrac{b^2}{a})\|u\|^2, 
  %    \)
  %    which is positive owing to \eqref{eq:elicit:lin:theta}. 
     
  %    %  \begin{align*}
  %    %   \langle v, A^\top u \rangle 
  %    %    {}={}
  %    %  \langle v, \proj_{X}\big(A^\top \proj_{X^\bot}(u)\big) \rangle 
  %    %    {}\geq{}
  %    %  -b_4\|u\|\|v\|. 
  %    % \end{align*}
  %   %   We proceed by lower bounding the inner products above through repeated use of the Fenchel-Young inequality. We have 
  %   % \begin{align*}
  %   %   \langle u, Au \rangle 
  %   %     {}={}
  %   %   \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   - \tfrac{\varepsilon_1}{2}b_1^2\|u\|^2
  %   %   - \tfrac{1}{2\varepsilon_1}\|u\|^2,    
  %   %  \end{align*} 
  %   %  where the equality follows by orthogonality between \(X\) and \(X^\bot\). 
  %   %  Similarly, 
  %   %  \begin{align*}
  %   %    \langle v, (A+A^\top)u \rangle 
  %   %     {}={}
  %   %   \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   -\tfrac{\varepsilon_2}{2}b_2^2\|u\|^2 -  \tfrac{1}{2\varepsilon_2} \|v\|^2,    
  %   %  \end{align*}
  %   %  \begin{align*}
  %   %    \langle v, A^\top A u \rangle 
  %   %     {}={}
  %   %   \langle v, \proj_{X}\big(A^\top A\proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   -\tfrac{\varepsilon_3}{2}b_3^2\|u\|^2 - \tfrac{1}{2\varepsilon_3}\|v\|^2,
  %   %  \end{align*}
  %   %   \begin{align*}
  %   %    \langle v, A^\top u \rangle 
  %   %     {}={}
  %   %   \langle v, \proj_{X}\big(A^\top \proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   -\tfrac{\varepsilon_4}{2}b_4^2\|u\|^2 - \tfrac{1}{2\varepsilon_4}\|v\|^2,
  %   %  \end{align*}
  
  % \end{proof}
  % \end{lemma}

==> TeX/Text/deprecated/elication.tex <==

% \begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin:2}
%   Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
%   \begin{equation}\label{eq:PIlemlin:X:2}
%     \langle x, Ax \rangle 
%       {}\geq{}
%     \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
%   \end{equation}  
%   Let \(b_i= \|B_i\|\), \(i=1,2,3\), where the matrices \(\alpha,B_2,B_3\in\R^{n\times n}\) are defined by 
%   \begin{align*}
%     \alphaw
%       {}\coloneqq{}&
%     \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
%     \quad
%     B_2w
%       {}\coloneqq{}
%     \proj_{X}\big(A\proj_{X^\bot}(w)\big),
%     \quad
%     B_3w
%       {}\coloneqq{}
%     \proj_{X}\big(Aw\big),  \quad w \in \R^n.
%     % \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
%   \end{align*}
%   Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). Suppose that $\nuP \leq 0$ Then, 
%   % \(T^X\) is \(V\)-oblique comonotone if
%   \begin{enumerate}
%     \item If \(\rho_{A,X}>0\), then \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
%     \begin{align}
%       c
%         {}\geq{}
%        0, \quad  
%       % \label{eq:elicit:lin:rho}
%       % \\
%       0
%         {}\leq{}
%         \sigma_{A,X}-\nuPb_3^2 - \tfrac{b^2_2}{4c}
%       \label{eq:PIlemlin:theta:2}
%     \end{align}
%     where $c \dfn \theta-\nuD-\nuPb_3^2-\tfrac{1}{4\rho_{A,X}}-\alpha$.
%     \item If \(\rho_{A,X}=0\), \bhl{TODO}
%   \end{enumerate}
%   \bhl{Note: Here, we dealt with the final term through the introduction of $b_3$, allowing for potentially negative $\sigma_{A,X}$. However, it still isn't nice...}
%   \begin{proof}
%     Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
%   \begin{align*}
%     V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\langle w,\proj_{X^{\bot}}(w)\rangle - \nuP\|\proj_{X}(Aw)\|^{2}
%        {}\geq{}&
%      0.
%   \end{align*}
%   The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This implies that 
%   \(
%     \|w\|^2 
%       {}={}
%     \|v\|^2 + \|u\|^2,
%   \)
%   and
%   \begin{align*}
%     \langle w,Aw\rangle
%       {}={}&
%     \langle u+v,A(u+v)\rangle 
%     \\
%       {}={}&
%     % \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
%     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle
%   \end{align*}
%   First, consider the case when \(\rho_{A,X} > 0\). Then, it follows that
%   \begin{align*}
%     V(w)
%       {}={}&
%     % \langle v,Av\rangle + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
%     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
%     % \dueto{$(\nuP \leq 0)$}
%       {}\geq{}&
%       % \langle v,Av\rangle + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2\\
%       \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 \textcolor{red}{- \nuPb_3^2\|w\|^{2}}\\
%     \dueto{\eqref{eq:elicit:lin:X}}
%       {}\geq{}&
%       % \sigma_{A,X} \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2
%       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD-\nuPb_3^2)\|u\|^2\\
%       {}\geq{}&
%       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,Au\rangle - \tfrac{\varepsilon}{2}\|Av\|^2 - \tfrac{1}{2\varepsilon}\|u\|^2+ (\theta-\nuD-\nuPb_3^2)\|u\|^2
%   \end{align*}
%   where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle u, Av \rangle\). Setting $\varepsilon = 2\rho_{A,X} > 0$ yields
%   \begin{align*}
%     V(w)
%       {}\geq{}&
%       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 + \langle u,Au\rangle + \langle v,Au\rangle + (\theta-\nuD-\nuPb_3^2 - \tfrac{1}{4\rho_{A,X}})\|u\|^2
%       \numberthis \label{eq:PIlemlin:ineq:2}
%   \end{align*}

%   We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality.
%   \begin{align*}
%     \langle u, Au \rangle 
%       {}={}
%     \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
%       {}\geq{}
%     - \alpha\|u\|^2   
%     \numberthis \label{eq:PIlemlin:b1:2}
%    \end{align*} 
%    where the equality follows by orthogonality between \(X\) and \(X^\bot\). Similarly,
%   %  \begin{align*}
%   %   \langle v, (A+A^\top)u \rangle 
%   %    {}={}
%   %  \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
%   %    {}\geq{}
%   %  -b_2\|u\|\|v\|,    
%   % %  \numberthis \label{eq:elicit:lin:b2}
%   % \end{align*}
%   \begin{align*}
%     \langle v, Au \rangle 
%       {}={}
%     \langle v, \proj_{X}\big(A\proj_{X^\bot}(u)\big) \rangle 
%       {}\geq{}
%       -b_2\|u\|\|v\|. 
%     \numberthis \label{eq:PIlemlin:b2:2}
%    \end{align*} 
%    Using ~\eqref{eq:PIlemlin:b1:2} and~\eqref{eq:PIlemlin:b2:2} to lower bound~\eqref{eq:PIlemlin:ineq:2} yields
%    \begin{align*}
%     V(w)
%       {}\geq{}&
%       (\sigma_{A,X}-\nuPb_3^2) \|v\|^2 - b_2\|u\|\|v\| + c\|u\|^2
%   \end{align*}
%   where
%    \(
%       c 
%         {}\coloneqq{}
%       \theta-\nuD-\nuPb_3^2-\tfrac{1}{4\rho_{A,X}}-\alpha
%    \). 
%    Assuming $c \geq 0$ as in~\eqref{eq:PIlemlin:theta:2}, and using the Fenchel-Young inequality we obtain
%    \(
%     V(w) \geq (\sigma_{A,X}-\nuPb_3^2 - \tfrac{b^2_2}{4c})\|v\|^2, 
%    \)
%    which is positive owing to~\eqref{eq:PIlemlin:theta:2}. 
%   \end{proof}
% \end{lemma}

% \begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin:3}
%   Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
%   \begin{equation}\label{eq:PIlemlin:X:3}
%     \langle x, Ax \rangle 
%       {}\geq{}
%     \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
%   \end{equation}  
%   Let \(b_i= \|B_i\|\), \(i=1,2\), where the matrices \(\alpha,B_2\in\R^{n\times n}\) are defined by 
%   \begin{align*}
%     \alphaw
%       {}\coloneqq{}&
%     \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
%     \qquad
%     B_2w
%       {}\coloneqq{}
%     \proj_{X}\big(A\proj_{X^\bot}(w)\big),  \qquad w \in \R^n.
%     % \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
%   \end{align*}
%   Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). Suppose that $\nuP \leq 0$ Then, 
%   % \(T^X\) is \(V\)-oblique comonotone if
%   \begin{enumerate}
%     \item If \(\rho_{A,X}>0\), then \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
%     \begin{align}
%       c
%         {}\geq{}
%        0, \quad  
%       % \label{eq:elicit:lin:rho}
%       % \\
%       0
%         {}\leq{}
%      \sigma_{A,X} - \tfrac{b^2_2}{4c}
%       \label{eq:PIlemlin:theta:3}
%     \end{align}
%     where $c \dfn \theta-\nuD-\tfrac{1}{4\rho_{A,X}}-\alpha$.
%     \item If \(\rho_{A,X}=0\), \bhl{TODO}
%   \end{enumerate}
%   \begin{proof}
%     Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
%   \begin{align*}
%     V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\langle w,\proj_{X^{\bot}}(w)\rangle - \nuP\|\proj_{X}(Aw)\|^{2}
%        {}\geq{}&
%      0.
%   \end{align*}
%   The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This implies that 
%   \(
%     \|w\|^2 
%       {}={}
%     \|v\|^2 + \|u\|^2,
%   \)
%   and
%   \begin{align*}
%     \langle w,Aw\rangle
%       {}={}&
%     \langle u+v,Aw\rangle 
%     \\
%       {}={}&
%     % \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
%     \langle v,Aw\rangle+\langle u,A u\rangle+\langle u,Av\rangle
%   \end{align*}
%   First, consider the case when \(\rho_{A,X} > 0\). Then, it follows that
%   \begin{align*}
%     V(w)
%       {}={}&
%     \langle v,Aw\rangle+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
%       {}={}&
%       \langle v,\proj_X(Aw)\rangle+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
%       {}\geq{}&
%       - \tfrac{1}{2\varepsilon}\|v\|^2 - \tfrac{\varepsilon}{2}\|\proj_X(Aw)\|^2+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}
%   \end{align*}
%   where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle v,\proj_X(Aw)\rangle\). Setting $\varepsilon = -2\nuP > 0$ yields
%   \begin{align*}
%     V(w)
%       {}\geq{}&
%       \tfrac{1}{4\nuP}\|v\|^2+\langle u,A u\rangle+\langle u,Av\rangle + (\theta-\nuD)\|u\|^2
%   \end{align*}
%   ???
%   \end{proof}
% \end{lemma}

% \begin{lemma}[Comonotonicity of the partial inverse operator: linear case] \label{lem:partialinverse:comon:lin:3}
%   Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
%   \begin{equation}\label{eq:PIlemlin:X:3}
%     \langle x, Ax \rangle 
%       {}\geq{}
%     \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
%   \end{equation}  
%   Let \(b_i= \|B_i\|\), \(i=1,2\), where the matrices \(\alpha,B_2\in\R^{n\times n}\) are defined by 
%   \begin{align*}
%     \alphaw
%       {}\coloneqq{}&
%     \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
%     \qquad
%     B_2w
%       {}\coloneqq{}
%     \proj_{X}\big(A\proj_{X^\bot}(w)\big),  \qquad w \in \R^n.
%     % \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
%   \end{align*}
%   Set \( T = A + \theta \proj_{X^\bot}\) and let \(V = \nuP \proj_{X} + \nuD\proj_{X^\bot}\) for some \(\nuP,\nuD\in\R\). Suppose that $\nuP \leq 0$ Then, 
%   % \(T^X\) is \(V\)-oblique comonotone if
%   \begin{enumerate}
%     \item If \(\rho_{A,X}>0\), then \(T^X\) has elicitable \(V\)-oblique comonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
%     \begin{align}
%       c \dfn \theta-\nuD - \tfrac{1}{8\rho_{A,X}} - \alpha
%         {}\geq{}
%        0, \quad  
%       % \label{eq:elicit:lin:rho}
%       % \\
%       0
%         {}\leq{}
%       2\sigma_{A,X}+ \tfrac{1}{4\nuP} - \tfrac{b^2_2}{4c}
%       \label{eq:PIlemlin:theta:3}
%     \end{align}
%     where $c \dfn \theta-\nuD-\tfrac{1}{4\rho_{A,X}}-\alpha$.
%     \item If \(\rho_{A,X}=0\), \bhl{TODO}
%   \end{enumerate}
%   \begin{proof}
%     Leveraging~\eqref{eq:PIlem:cond} and linearity of the mapping $A$, it suffices to show that for all \(w\in\R^n\) the following holds: %\((x,y)\in\graph S\) for some \(\nuP,\nuD\)
%   \begin{align*}
%     V(w) \coloneqq \langle w,Aw\rangle+(\theta-\nuD)\langle w,\proj_{X^{\bot}}(w)\rangle - \nuP\|\proj_{X}(Aw)\|^{2}
%        {}\geq{}&
%      0.
%   \end{align*}
%   The vector \(w\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This implies that 
%   \(
%     \|w\|^2 
%       {}={}
%     \|v\|^2 + \|u\|^2,
%   \)
%   and
%   \begin{align*}
%     \langle w,Aw\rangle
%       {}={}&
%     \langle u+v,A(u+v)\rangle 
%     \\
%       {}={}&
%     % \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
%     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle
%   \end{align*}
%   First, consider the case when \(\rho_{A,X} > 0\). Then, it follows that
%   \begin{align*}
%     V(w)
%       {}={}&
%       \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 - \nuP\|\proj_{X}(Aw)\|^{2}\\
%       {}\geq{}&
%       \langle v,Av\rangle+\langle u,A u\rangle+\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 + \langle v,\proj_{X}(Aw)\rangle + \tfrac{1}{4\nuP}\|v\|^{2}
%   \end{align*}
%   where the Fenchel-Young inequality was used to control the inner product \(\langle v,\proj_X(Aw)\rangle\). Since $\langle v,\proj_{X}(Aw)\rangle = \langle v,Aw\rangle$, it follows that
%   \begin{align*}
%     V(w)
%       {}\geq{}&
%       2\langle v,Av\rangle+\langle u,A u\rangle+2\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2 + \tfrac{1}{4\nuP}\|v\|^{2}\\
%     \dueto{\eqref{eq:elicit:lin:X}}
%       {}\geq{}&
%       % \sigma_{A,X} \|v\|^2 + \rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + \langle v,(A+A^{\top})u\rangle + (\theta-\nuD)\|u\|^2
%       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 + 2\rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + 2\langle v,Au\rangle + \langle u,Av\rangle + (\theta-\nuD)\|u\|^2\\
%       {}\geq{}&
%       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 + 2\rho_{A,X}\|Av\|^2 + \langle u,Au\rangle + 2\langle v,Au\rangle - \tfrac{\varepsilon}{2}\|Av\|^2 - \tfrac{1}{2\varepsilon}\|u\|^2+ (\theta-\nuD)\|u\|^2
%   \end{align*}
%   where the Fenchel-Young inequality was used in the last inequality to control the inner product \(\langle u, Av \rangle\). Setting $\varepsilon = 4\rho_{A,X} > 0$ yields
%   \begin{align*}
%     V(w)
%       {}\geq{}&
%       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 + \langle u,Au\rangle + 2\langle v,Au\rangle + (\theta-\nuD - \tfrac{1}{8\rho_{A,X}})\|u\|^2
%       \numberthis \label{eq:PIlemlin:ineq:3}
%   \end{align*}

%   We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality.
%   \begin{align*}
%     \langle u, Au \rangle 
%       {}={}
%     \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
%       {}\geq{}
%     - \alpha\|u\|^2   
%     \numberthis \label{eq:PIlemlin:b1:3}
%    \end{align*} 
%    where the equality follows by orthogonality between \(X\) and \(X^\bot\). Similarly,
%   %  \begin{align*}
%   %   \langle v, (A+A^\top)u \rangle 
%   %    {}={}
%   %  \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
%   %    {}\geq{}
%   %  -b_2\|u\|\|v\|,    
%   % %  \numberthis \label{eq:elicit:lin:b2}
%   % \end{align*}
%   \begin{align*}
%     \langle v, Au \rangle 
%       {}={}
%     \langle v, \proj_{X}\big(A\proj_{X^\bot}(u)\big) \rangle 
%       {}\geq{}
%       -b_2\|u\|\|v\|. 
%     \numberthis \label{eq:PIlemlin:b2:3}
%    \end{align*} 
%    Using ~\eqref{eq:PIlemlin:b1:3} and~\eqref{eq:PIlemlin:b2:3} to lower bound~\eqref{eq:PIlemlin:ineq:3} yields
%    \begin{align*}
%     V(w)
%       {}\geq{}&
%       (2\sigma_{A,X}+ \tfrac{1}{4\nuP}) \|v\|^2 - b_2\|u\|\|v\| + c\|u\|^2
%   \end{align*}
%   where
%    \(
%       c 
%         {}\coloneqq{}
%       \theta-\nuD - \tfrac{1}{8\rho_{A,X}} - \alpha
%    \). 
%    Assuming $c \geq 0$ as in~\eqref{eq:PIlemlin:theta:3}, and using the Fenchel-Young inequality we obtain
%    \(
%     V(w) \geq (2\sigma_{A,X}+ \tfrac{1}{4\nuP} - \tfrac{b^2_2}{4c})\|v\|^2, 
%    \)
%    which is positive owing to~\eqref{eq:PIlemlin:theta:3}. 
%   \end{proof}
% \end{lemma}

\bhl{TODO: the remainder of this note contains old results which might be relevant, need to fix refs}
The general inclusion problem \eqref{eq:DRS problem} may be equivalently cast as a linkage problem by introducing auxiliary variables as follows. 
\begin{align*}
	0 
		{}\in{}
	Ax_1 + B x_1
		{}\iff{}&
	0 
		{}\in{}
	Ax_1 + y_2,
	\quad
	0
		{}\in{}
	Bx_1 - y_2
	\\
	{}\iff{}&
	x= (x_1,x_2)
		{}\in{}
	X,
	\quad
	y=(y_1,y_2) 
		{}\in{}
	X^\bot
	,\quad 
	y
		{}\in{}
	{\hat T}x,
\end{align*}
where 
\[
	\hat T x
		{}={}
	(Ax_1, Bx_2),
	\quad 
	X= \set{x=(x_1,x_2)\in \R^{2n}}[x_1 = x_2]. 
\]
Leveraging the idea of elicitation, operator \(\hat T\) in the above inclusion above may be replaced by \({\hat T}x + \theta \proj_{X^\bot}(x)\) for any \(\theta \in[0,\infty)\) without affecting the solutions of the inclusion. 
Further noting that 
\(
	\proj_X(x) = \big(\tfrac12 (x_1 + x_2), \tfrac12 (x_1 + x_2) \big),
\)
leads to the following equivalent problem 
\[
	x= (x_1,x_2)
	{}\in{}
	X,
	\quad
	y=(y_1,y_2) 
	{}\in{}
	X^\bot
	,\quad 
	y
	{}\in{}
	\left(%
	Ax_{1} + \tfrac{\theta}{2}(x_{1}+x_{2}), 
	Bx_{2}  + \tfrac{\theta}{2}(x_{1}+x_{2})
	\right).
\]


\hl{TODO: Elicitation preliminaries}

\begin{lemma}\label{lem:elicit:linear}
    Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\) for some \(\rho_{A,X}\geq0\) and \(\sigma_{A,X}\in\R^n\), \ie, 
    \begin{equation}\label{eq:elicit:lin:X}
        \langle Ax, x \rangle 
          {}\geq{}
        \sigma_{A,X} \|x\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
      \end{equation}  
    Let \(b_i= \|B_i\|\), \(i=1,2\), where the matrices \(B_1,B_2\in\R^{n\times n}\) are defined by 
	\begin{align*}
		B_1w
			{}\coloneqq{}&
		\proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
		\qquad
		B_2w
			{}\coloneqq{}
		\proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big), \qquad w \in \R^n.
	\end{align*}
	Suppose that \(\sigma_A < \sigma_{A,X}\). Then,
	\begin{enumerate}
		\item If \(\rho_{A,X}>0\), then \(A\) has elicitable \((\sigma_A,\rho_A)\)-semimonotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
		\begin{align}
		\rho_A 
			{}\leq{}
		0, \quad  
		% \label{eq:elicit:lin:rho}
		% \\
		0
			{}\leq{}
		-\rho_{A}\left(1+\tfrac{\rho_{A}}{\rho_{A,X}}\right)\theta^{2}
			{}+{}
		(1+2\rho_{A}b_{1})\theta
			{}+{}
		\tfrac{b_{2}^{2}}{4\sigma_{A}^{\prime}}-\sigma_{A}-b_{1}
		\label{eq:elicit:lin:theta}
		\end{align}
		\item If \(\rho_{A,X}=0\) then \(A\) has elicitable \((\sigma_A,0)\)-semimonotonicity (everywhere) at level \(\theta \geq \sigma_A + b_1 + \tfrac{b_2^2}{4(\sigma_{A,X}-\sigma_A)}\). 
	\end{enumerate}
	\begin{proof}
		A given vector \(w\in\R^n\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This would imply that 
		\(
			\|w\|^2 
			{}={}
			\|v\|^2 + \|u\|^2,
		\)
		and 
		\begin{align*}
			\|Aw+\theta\proj_{X^{\top}}(w)\|^{2}
			{}={}&
			\|Aw\|^{2}+\theta^{2}\|\proj_{X^{\top}}(w)\|^{2}+2\langle Aw,\theta\proj_{X^{\top}}(w)\rangle
			\\
			{}={}&
			\|Aw\|^{2}+\theta^{2}\|u\|^{2}+2\theta\langle Av+Au,u\rangle.
			\numberthis \label{eq:elicit:1}
		\end{align*}
		The mapping \(A+ \theta \proj_{X^\bot}\) is linear. Therefore, to establish the claim it suffices to show that for all \(w\in\R^n\) the following holds for some \(\rho_A, \sigma_A\leq0\):
		\begin{align*}
			V(w) \coloneqq \langle w,Aw+\theta\proj_{X^{\top}}(w)\rangle-\sigma_{A}\|w\|^{2} - \rho_{A}\|Aw+\theta\proj_{X^{\top}}(w)\|^{2} \geq 0. 
		\end{align*}
		Note that 
		\begin{align*}
			\langle w,Aw+\theta \proj_{X^\bot}(w)\rangle
			{}={}&
			\langle u+v,A(u+v)+\theta u\rangle 
			\\
			{}={}&
			\langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
			{}+{}
			\theta \|u\|^2
		\end{align*}
		First, consider the case when \(\rho_{A,X} > 0\). Combine this with \eqref{eq:elicit:1} to obtain
		\begin{align*}
			V(w) 
			{}={}&
			\langle v,Av\rangle-\sigma_{A}\|v\|^{2}-\rho_{A}\|Aw\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
			\\%
			&{}+{}
			\langle v,(A+A^{\top})u\rangle 
			{}+{}
			(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle
			\numberthis\label{eq:elicit:lin:Aw}
			\\%
			\dueto{\eqref{eq:elicit:lin:X}}
			{}\geq{}&
			-\sigma_{A}^\prime\|v\|^{2}+\rho_{A,X}\|Av\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
			\\%
			&{}+{}
			\langle v,(A+A^{\top})u\rangle 
			{}+{}
			(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle Av,u\rangle  
			\\%
				{}\geq{}&
			-\sigma_{A}^\prime\|v\|^{2}
			{}+{}
			\rho_{A,X}\|Av\|^{2}
			{}+{}
			(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
			\\%
			&{}+{}
			\langle v,(A+A^{\top})u\rangle
			{}+{}
			(1-2\rho_{A}\theta)\langle Au,u\rangle+ \tfrac{\rho_{A}\theta}{\varepsilon} \|Av\|^2 + \rho_{A}\theta \varepsilon \|u\|^2  
		\end{align*}
		where \(\sigma_{A}^\prime = \sigma_{A} - \sigma_{A,X}\) and the Fenchel-young inequality was used in the last inequality to control the inner product \(-2\rho_A\theta\langle Av,u \rangle\). 
		Setting \(\varepsilon = -\tfrac{\rho_A \theta}{\rho_{A,X}}>0\) yields 
		\begin{align*}
			V(w) 
			{}={}&
			-\sigma_{A}^\prime\|v\|^{2}
				{}+{}
			\big(%
				\theta-\sigma_{A}-\rho_{A}\theta^{2} - \tfrac{\rho_{A}^2\theta^2}{\rho_{A,X}}
			\big)\|u\|^{2}
			\\%
				&{}+{}
			\langle v,(A+A^{\top})u\rangle
				{}+{}
			(1-2\rho_{A}\theta)\langle Au,u\rangle 
			\numberthis\label{eq:elicit:lin:Vw}
		\end{align*}
		We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality. 
		\begin{align*}
		\langle u, Au \rangle 
			{}={}
		\langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
			{}\geq{}
		- b_1\|u\|^2   
		\numberthis \label{eq:elicit:lin:b1}
		\end{align*} 
		where the equality follows by orthogonality between \(X\) and \(X^\bot\). 
		Similarly, 
		\begin{align*}
		\langle v, (A+A^\top)u \rangle 
			{}={}
		\langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
			{}\geq{}
		-b_2\|u\|\|v\|,    
		\numberthis \label{eq:elicit:lin:b2}
		\end{align*}
		Using \eqref{eq:elicit:lin:b1}, \eqref{eq:elicit:lin:b2} to lower bound \eqref{eq:elicit:lin:Vw} yields
		\begin{align*}
		V(w) 
			{}\geq{}&
		-\sigma_A^\prime\|v\|^{2} - b_2\|u\|\|v\| + c\|u\|^2
		\end{align*}
		where
		\(
		c 
			{}\coloneqq{}
		\theta-\sigma_{A}-\rho_{A}\theta^{2} - \tfrac{\rho_{A}^2\theta^2}{\rho_{A,X}} -(1-2\rho_{A}\theta)b_{1}
		\). 
		Further noting that \(\sigma_{A}^{\prime}<0\), \(\rho_A\leq0\) as ensured in \eqref{eq:elicit:lin:theta}, and using the Fenchel-Young inequality we obtain
		\(
		V(w) \geq (c + \tfrac{b^2_2}{4\sigma_A^\prime})\|u\|^2, 
		\)
		which is positive owing to \eqref{eq:elicit:lin:theta}. 
		
		In the case where \(\rho_{A,X} = 0\), \eqref{eq:elicit:lin:Aw} simplifies to 
		\begin{align*}
		V(w) 
			{}={}&
		\langle v,Av\rangle-\sigma_{A}\|v\|^{2}+(\theta-\sigma_{A})\|u\|^{2}
		% \\%
			{}+{}
		\langle v,(A+A^{\top})u\rangle 
			{}+{}
		\langle Au,u\rangle.
		\end{align*}
		Following the same steps as above yields the claimed range for \(\theta\). 

		\bhl{Could we have used the positive terms \(\|Aw\|^2\) in \eqref{eq:elicit:lin:Aw} to obtain a better parameter range?}
	\end{proof}
\end{lemma}
  
  
  % \begin{lemma}
  %     Let \(X\subseteq \R^n\) be a closed linear subspace. Suppose that \(A\in\R^{n\times n}\) is a linear mapping such that \(A\) is \((\sigma_{A,X}, \rho_{A,X})\)-semimonotone relative to \(X\), \ie, 
  %     \begin{equation}\label{eq:elicit:lin:X}
  %         \langle Ax, x \rangle 
  %           {}\geq{}
  %         \sigma_{A,X} \|w\|^2 + \rho_{A,X}\|Ax\|^2,\quad x\in X.  
  %       \end{equation}  
  %     Then, \(A\) has elicitable \((\sigma_A,\rho_A)\)-semi-monotonicity (everywhere) at the level \(\theta\in[0,\infty)\) satisfying 
  % \begin{align}
  %   \rho_A 
  %     {}\leq{}&
  %    0, \quad \rho_{A}\leq \rho_{A,X}, 
  %   % \\
  %   \quad
  %   % \sigma_{A}^\prime
  %     % {}={}
  %   \sigma_{A} 
  %     {}<{}
  %   \sigma_{A,X},  
  %   \label{eq:elicit:lin:rho}
  %   % \label{eq:elicit:lin:sigma}
  %   \\
  %   0
  %     {}\leq{}&
  %  \left(\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}\right)
  %     {}+{}
  %   \tfrac{1}{(\sigma_{A}-\sigma_{A,X})}\left(\rho_{A}\theta b_{4}+\rho_{A}b_{3}-\tfrac{1}{2}b_{2}\right)^{2}
  %   \label{eq:elicit:lin:theta}
  % \end{align}
  % \hl{TODO: a clean range for theta?...}
  
  % where \(b_i= \|B_i\|\), \(i=1,\cdots,4\), and the matrices 
  %  \(B_1,B_2,B_3,B_4\in\R^{n\times n}\) are define by 
  % \begin{align*}
  %   B_1w 
  %     {}\coloneqq{}&
  %   \proj_{X^\bot}\big(A\proj_{X^\bot}(w)\big),
  %   \qquad
  %   B_2w 
  %     {}\coloneqq{}
  %   \proj_{X}\big((A+A^\top)\proj_{X^\bot}(w)\big),
  %     \\
  %   B_3w 
  %     {}\coloneqq{}&
  %   \proj_{X}\big((A^\top A)\proj_{X^\bot}(w)\big),
  %   \quad
  %   B_4w 
  %     {}\coloneqq{}
  %   \proj_{X}\big(A^\top \proj_{X^\bot}(w)\big).
  % \end{align*}
  % In particular, if \(\rho_{A,X}=0\) then \(A\) has elicitable \((\sigma_A,0)\)-semi-monotone at level \(\theta \geq \sigma_A + b_1 + \tfrac{b_2^2}{4(\sigma_{A,X}-\sigma_A)}\). 
  % \begin{proof}
  %   A given vector \(w\in\R^n\) may be represented as the sum of elements of \(X\) and its orthogonal complement \(X^\bot\), \ie,  \(w = v + u \) where \(v = \proj_X(w)\) and \(u= \proj_{X^\bot}(w)\). This would imply that 
  %   \(
  %     \|w\|^2 
  %       {}={}
  %     \|v\|^2 + \|u\|^2,
  %   \)
  %   and 
  %   \begin{align*}
  %     \|Aw+\theta\proj_{X^{\top}}(w)\|^{2}
  %       {}={}&
  %     \|Aw\|^{2}+\theta^{2}\|\proj_{X^{\top}}(w)\|^{2}+2\langle Aw,\theta\proj_{X^{\top}}(w)\rangle
  %     \\
  %       {}={}&
  %     \|Av\|^{2}+\|Au\|^{2}+2\langle Av,Au\rangle+\theta^{2}\|u\|^{2}+2\theta\langle Av+Au,u\rangle.
  %     \numberthis \label{eq:elicit:1}
  %   \end{align*}
  %   The mapping \(A+ \theta \proj_{X^\bot}\) is linear. Therefore, to establish the claim it suffices to show that for all \(w\in\R^n\) the following holds for some \(\rho_A, \sigma_A\leq0\). 
  %   \begin{align*}
  %     V(w) \coloneqq \langle w,Aw+\theta\proj_{X^{\top}}(w)\rangle-\sigma_{A}\|w\|^{2} - \rho_{A}\|Aw+\theta\proj_{X^{\top}}(w)\|^{2} \geq 0. 
  %   \end{align*}
  %   Note that 
  %   \begin{align*}
  %     \langle w,Aw+\theta \proj_{X^\bot}(w)\rangle
  %       {}={}&
  %     \langle u+v,A(u+v)+\theta u\rangle 
  %     \\
  %       {}={}&
  %     \langle v,Av\rangle+\langle u,A u\rangle+\langle v,(A+A^{\top})u\rangle
  %       {}+{}
  %     \theta \|u\|^2
  %   \end{align*}
  %   Combine this with \eqref{eq:elicit:1} to obtain
  %   \begin{align*}
  %     V(w) 
  %       {}={}&
  %     \langle v,Av\rangle-\sigma_{A}\|v\|^{2}-\rho_{A}\|Av\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}-\rho_{A}\|Au\|^{2}
  %     \\%
  %       &{}+{}
  %     \langle v,(A+A^{\top})u\rangle-2\rho_{A}\langle v,A^{\top}Au\rangle+(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle
  %     \\%
  %     \dueto{\eqref{eq:elicit:lin:X}}
  %       {}\geq{}&
  %     -\sigma_{A}^\prime\|v\|^{2}-\rho_{A}^\prime\|Av\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}-\rho_{A}\|Au\|^{2}
  %     \\%
  %       &{}+{}
  %     \langle v,(A+A^{\top})u\rangle-2\rho_{A}\langle v,A^{\top}Au\rangle+(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle  
  %     \\%
  %         {}\geq{}&
  %     -\sigma_{A}^\prime\|v\|^{2}+(\theta-\sigma_{A}-\rho_{A}\theta^{2})\|u\|^{2}
  %     \\%
  %       &{}+{}
  %     \langle v,(A+A^{\top})u\rangle-2\rho_{A}\langle v,A^{\top}Au\rangle+(1-2\rho_{A}\theta)\langle Au,u\rangle-2\rho_{A}\theta\langle v,A^{\top}u\rangle  
  %     \numberthis\label{eq:elicit:lin:Vw}
  %   \end{align*}
  %   where \(\sigma_{A}^\prime = \sigma_{A} - \sigma_{A,X}\) and \(\rho_{A}^\prime =\rho_{A} - \rho_{A,X}\), and \eqref{eq:elicit:lin:rho} was used in the last inequality. 
  
  %   We proceed by lower bounding the inner products above through repeated use of the Cauchy-Schwarz inequality. 
  %   \begin{align*}
  %     \langle u, Au \rangle 
  %       {}={}
  %     \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     - b_1\|u\|^2   
  %     \numberthis \label{eq:elicit:lin:b1}
  %    \end{align*} 
  %    where the equality follows by orthogonality between \(X\) and \(X^\bot\). 
  %    Similarly, 
  %    \begin{align*}
  %      \langle v, (A+A^\top)u \rangle 
  %       {}={}
  %     \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     -b_2\|u\|\|v\|,    
  %     \numberthis \label{eq:elicit:lin:b2}
  %    \end{align*}
  %    and 
  %    \begin{align*}
  %      \langle v, A^\top A u \rangle 
  %       % {}={}
  %     % \langle v, \proj_{X}\big(A^\top A\proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     -b_3\|u\|\|v\|,
  %     \quad 
  %     \langle v, A^\top u \rangle 
  %       % {}={}
  %     % \langle v, \proj_{X}\big(A^\top \proj_{X^\bot}(u)\big) \rangle 
  %       {}\geq{}
  %     -b_4\|u\|\|v\|. 
  %     \numberthis \label{eq:elicit:lin:b34}
  %    \end{align*}
  %    Using \eqref{eq:elicit:lin:b1}, \eqref{eq:elicit:lin:b2}, \eqref{eq:elicit:lin:b34} to lower bound \eqref{eq:elicit:lin:Vw} yields
  %    % \begin{align*}
  %    %  V(w) 
  %    %    {}\geq{}&
  %    %  -\sigma_{A}^{\prime}\|v\|^{2}+\left(2\rho_{A}\theta b_{4}+2\rho_{A}b_{3}-b_{2}\right)\|u\|\|v\|
  %    %  \\
  %    %    &{}+{}
  %    %  (\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1})\|u\|^{2} 
  %    %  \\
  %    %    {}\geq{}&
  %    %  \big(\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}\big)\|u\|^{2}
  %    % \end{align*}
  %    % 
  %     \begin{align*}
  %     V(w) 
  %       {}\geq{}&
  %     a\|v\|^{2} - 2b\|u\|\|v\| + c\|u\|^2
  %     \\
  %     %   {}\geq{}&
  %     % \big(\theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}\big)\|u\|^{2}
  %    \end{align*}
  %    where
  %    \[
  %     a \coloneqq -\sigma_A^\prime,
  %     \quad
  %     b \coloneqq -\rho_{A}\theta b_{4}-\rho_{A}b_{3} + \tfrac12b_{2}, 
  %     \quad
  %     c \coloneqq \theta-\sigma_{A}-\rho_{A}\theta^{2}-(1-2\rho_{A}\theta)b_{1}.
  %    \]
  %    Further noting that \(\sigma_{A}^{\prime}<0\), \(\rho_A\leq0\) as ensured in \eqref{eq:elicit:lin:rho}, and using the Fenchel-Young inequality we obtain
  %    \(
  %     V(w) \geq (c - \tfrac{b^2}{a})\|u\|^2, 
  %    \)
  %    which is positive owing to \eqref{eq:elicit:lin:theta}. 
     
  %    %  \begin{align*}
  %    %   \langle v, A^\top u \rangle 
  %    %    {}={}
  %    %  \langle v, \proj_{X}\big(A^\top \proj_{X^\bot}(u)\big) \rangle 
  %    %    {}\geq{}
  %    %  -b_4\|u\|\|v\|. 
  %    % \end{align*}
  %   %   We proceed by lower bounding the inner products above through repeated use of the Fenchel-Young inequality. We have 
  %   % \begin{align*}
  %   %   \langle u, Au \rangle 
  %   %     {}={}
  %   %   \langle u, \proj_{X^\bot}\big(A\proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   - \tfrac{\varepsilon_1}{2}b_1^2\|u\|^2
  %   %   - \tfrac{1}{2\varepsilon_1}\|u\|^2,    
  %   %  \end{align*} 
  %   %  where the equality follows by orthogonality between \(X\) and \(X^\bot\). 
  %   %  Similarly, 
  %   %  \begin{align*}
  %   %    \langle v, (A+A^\top)u \rangle 
  %   %     {}={}
  %   %   \langle v, \proj_{X}\big((A+A^\top)\proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   -\tfrac{\varepsilon_2}{2}b_2^2\|u\|^2 -  \tfrac{1}{2\varepsilon_2} \|v\|^2,    
  %   %  \end{align*}
  %   %  \begin{align*}
  %   %    \langle v, A^\top A u \rangle 
  %   %     {}={}
  %   %   \langle v, \proj_{X}\big(A^\top A\proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   -\tfrac{\varepsilon_3}{2}b_3^2\|u\|^2 - \tfrac{1}{2\varepsilon_3}\|v\|^2,
  %   %  \end{align*}
  %   %   \begin{align*}
  %   %    \langle v, A^\top u \rangle 
  %   %     {}={}
  %   %   \langle v, \proj_{X}\big(A^\top \proj_{X^\bot}(u)\big) \rangle 
  %   %     {}\geq{}
  %   %   -\tfrac{\varepsilon_4}{2}b_4^2\|u\|^2 - \tfrac{1}{2\varepsilon_4}\|v\|^2,
  %   %  \end{align*}
  
  % \end{proof}
  % \end{lemma}
